Computing Graph Descriptors on Edge Streams

Feature extraction is an essential task in graph analytics. These feature vectors, called graph descriptors, are used in downstream vector-space-based graph analysis models. This idea has proved fruitful in the past, with spectral-based graph descriptors providing state-of-the-art classification accuracy. However, known algorithms to compute meaningful descriptors do not scale to large graphs since: (1) they require storing the entire graph in memory, and (2) the end-user has no control over the algorithm's runtime. In this paper, we present streaming algorithms to approximately compute three different graph descriptors capturing the essential structure of graphs. Operating on edge streams allows us to avoid storing the entire graph in memory, and controlling the sample size enables us to keep the runtime of our algorithms within desired bounds. We demonstrate the efficacy of the proposed descriptors by analyzing the approximation error and classification accuracy. Our scalable algorithms compute descriptors of graphs with millions of edges within minutes. Moreover, these descriptors yield predictive accuracy comparable to the state-of-the-art methods but can be computed using only 25% as much memory.

==> heat.tex <==
x,t2,t3,t4
0.001,0.000992250439793453,8.152522773032092e-06,8.152522689955052e-06
0.002,0.0009897541946795605,9.468802044200773e-06,9.468800710035219e-06
0.003,0.000987258548495306,1.0786387927766465e-05,1.0786381135064007e-05
0.004,0.0009847650457177142,1.2105285853765461e-05,1.2105264286163853e-05
0.005,0.0009822752348101994,1.3425503402741626e-05,1.342545045080022e-05
0.006,0.00097978066753567,1.4747050502934716e-05,1.474693988016644e-05
0.007,0.000977302903618255,1.6069939213453553e-05,1.60697327862092e-05
0.008,0.0009748335009401093,1.7394184302596723e-05,1.7393829343560486e-05
0.009000000000000001,0.0009723740239562235,1.871980233321956e-05,1.871922968009312e-05
0.010000000000000002,0.000969926041131838,2.004681232191779e-05,2.0045933871512116e-05
0.011,0.0009674911249473018,2.1375235349501444e-05,2.13739419417359e-05
0.012,0.000965070851902183,2.270509537739241e-05,2.270325385555525e-05
0.013000000000000001,0.0009626668025207638,2.4036418395263597e-05,2.4033869521607255e-05
0.014000000000000002,0.0009602805613562853,2.5369232541036266e-05,2.5365788786698087e-05
0.015,0.00095791371699608,2.6703567251566023e-05,2.6699011432238778e-05
0.016,0.0009555578810040252,2.8039454651906943e-05,2.8033537170810092e-05
0.017,0.0009532346142240639,2.937692933439708e-05,2.9369365643149425e-05
0.018000000000000002,0.0009509355342787345,3.0716028162468135e-05,3.070649641477564e-05
0.019000000000000003,0.0009486622459398264,3.2056790278061855e-05,3.204492897251287e-05
0.02,0.0009464163580367775,3.339925710992694e-05,3.33846627216069e-05
0.021,0.0009441994834626412,3.474347238023175e-05,3.472569698141451e-05
0.022000000000000002,0.0009420132391775752,3.6089482683765746e-05,3.6068030983163335e-05
0.023,0.0009398592462144641,3.7437337859077115e-05,3.7411663865923515e-05
0.024,0.0009377391296835022,3.8787087077999474e-05,3.8756594673337814e-05
0.025,0.0009356545187771844,4.0138783380259215e-05,4.010282235011673e-05
0.026000000000000002,0.0009335970869159733,4.1492484708981524e-05,4.14503457387162e-05
0.027000000000000003,0.0009315883933966254,4.284824899907473e-05,4.279916357628101e-05
0.028,0.0009296201176363755,4.4206134542499385e-05,4.414927449024522e-05
0.029,0.0009276939052043875,4.5566203859781355e-05,4.550067699582078e-05
0.030000000000000002,0.000925811405776318,4.6928521841665246e-05,4.6853369491919266e-05
0.031,0.0009239742731386544,4.8293155757470235e-05,4.820735025812804e-05
0.032,0.0009222110090290928,4.966017526234454e-05,4.956261745066069e-05
0.033,0.0009205325204642092,5.1029652405785e-05,5.091916945247054e-05
0.034,0.0009189043054390246,5.240166163890136e-05,5.22770040067937e-05
0.035,0.0009173280298738631,5.3776279822755965e-05,5.363611891547668e-05
0.036000000000000004,0.0009157954464931826,5.5153586236106716e-05,5.4996511738422444e-05
0.037000000000000005,0.000914328066478457,5.653366258335894e-05,5.635817993818839e-05
0.038,0.0009129176484766895,5.7916593002412825e-05,5.7721120936961825e-05
0.039,0.0009115658749413846,5.930246407279536e-05,5.9085332029475414e-05
0.04,0.0009102744324715397,6.069136482335762e-05,6.0450810152849475e-05
0.041,0.000909060450540846,6.208338674036228e-05,6.18175522119372e-05
0.042,0.0009079374292694701,6.347862377551844e-05,6.31855549534737e-05
0.043000000000000003,0.000906879746331263,6.487717235383424e-05,6.455481496233589e-05
0.044000000000000004,0.0009058891019637108,6.627913138196917e-05,6.592532865820227e-05
0.045,0.0009049672005668215,6.768460225545751e-05,6.729709229115232e-05
0.046,0.0009041058775851793,6.9093688867749e-05,6.867010193893373e-05
0.047,0.0009033265945204647,7.050652412689285e-05,7.004435350250659e-05
0.048,0.000902621192662553,7.19231951946324e-05,7.141984270272291e-05
0.049,0.0009019913931078102,7.334381200271143e-05,7.279656683968528e-05
0.05,0.0009014389211389028,7.476848868045239e-05,7.417451996385325e-05
0.051000000000000004,0.000900965506229226,7.619734189887952e-05,7.555369701145131e-05
0.052000000000000005,0.0009005728820483751,7.763049087829572e-05,7.693409295917425e-05
0.053000000000000005,0.0009002627864666556,7.906805739661656e-05,7.831570258517691e-05
0.054,0.0009000369615597625,8.05101657977334e-05,7.969852046546404e-05
0.055,0.0008998971536140743,8.195694299914882e-05,8.108254096966172e-05
0.056,0.0008998352659480312,8.340851850067986e-05,8.246775825766104e-05
0.057,0.0008999000808952218,8.486502439230448e-05,8.385416627551914e-05
0.058,0.0009000606936535807,8.632659536209929e-05,8.524175875141847e-05
0.059000000000000004,0.0009003141312918504,8.779336870518088e-05,8.663052919242504e-05
0.060000000000000005,0.0009006621565409631,8.926548433094538e-05,8.802047087980718e-05
0.061,0.0009011065363612523,9.074308477217091e-05,8.941157686586327e-05
0.062,0.00090164904194799,9.222631519261281e-05,9.080383996958878e-05
0.063,0.000902291448736114,9.37153233953205e-05,9.219725277266879e-05
0.064,0.0009030355364045992,9.521025983137379e-05,9.359180795085588e-05
0.065,0.000903883088882041,9.671127760740434e-05,9.498749858046011e-05
0.066,0.0009048260942217493,9.821853249450106e-05,9.638431561335506e-05
0.067,0.0009058859479664313,9.973218293604027e-05,9.778225291439997e-05
0.068,0.0009070546438662922,0.00010125239005610704,9.918129953553536e-05
0.069,0.000908333982895133,0.00010277931766811588,0.00010058144657217071
0.07,0.0009097257703005746,0.00010431313228248687,0.00010198268485501668
0.07100000000000001,0.0009112318156084964,0.00010585400311547529,0.00010338500494641741
0.07200000000000001,0.0009128539326278866,0.00010740210209749302,0.0001047883971363134
0.07300000000000001,0.0009145939394560062,0.0001089576038811083,0.00010619285143787988
0.074,0.0009164536584829494,0.00011052068584974075,0.00010759835758374496
0.075,0.0009184349163967492,0.00011209152812576311,0.0001090049050216601
0.076,0.0009205297732525504,0.00011367031357921075,0.00011041248291066381
0.077,0.0009227596092324245,0.00011525722783590097,0.00011182108266075105
0.078,0.000925133830654394,0.00011685245928584698,0.00011323069493477545
0.079,0.0009276369104323493,0.0001184561990918349,0.00011464130391373592
0.08,0.0009302704981618526,0.00012006864119783379,0.00011605289758337285
0.081,0.0009330364428895877,0.0001216899823372756,0.0001174654636203417
0.082,0.0009359365979858613,0.00012332042204150353,0.00011887898938800644
0.083,0.0009389728211491484,0.000124960162648597,0.00012029346193252226
0.084,0.000942146974411315,0.00012660940931142164,0.00012170886797829824
0.085,0.0009454609241424824,0.00012826837000616634,0.00012312519392376805
0.08600000000000001,0.0009489068206542103,0.0001299372555412294,0.00012454242583749512
0.08700000000000001,0.0009525059829898054,0.00013161627956524005,0.0001259605494534786
0.08800000000000001,0.0009562505669990492,0.00013330565857581385,0.0001273795501670773
0.089,0.0009601424564530509,0.0001350056119281437,0.00012879941303074914
0.09,0.00096418353948538,0.0001367163618434147,0.00013022012274966065
0.091,0.0009683757085969067,0.00013843813341744902,0.000131641664669196
0.092,0.0009727208606607932,0.00014017115462911748,0.00013306403585336621
0.093,0.000977220896927137,0.0001419156563491544,0.00013448720682759783
0.094,0.0009818777230279905,0.00014367187234859096,0.0001359111608970963
0.095,0.0009866932489821776,0.00014544003930741923,0.00013733588099867208
0.096,0.0009916597013835424,0.00014722039682306284,0.00013876134969629286
0.097,0.000996798378027376,0.0001490131874193971,0.0001401875491769481
0.098,0.001002101510968342,0.00015081865655474584,0.00014161446124573304
0.099,0.0010075710278210637,0.00015263705263127676,0.00014304206732196993
0.1,0.0010132088606115796,0.00015446862700296916,0.00014447034843425698
0.101,0.0010190169457819026,0.00015631363398474523,0.00014589928521629406
0.10200000000000001,0.0010249972241948779,0.0001581723308610814,0.00014732885790237976
0.10300000000000001,0.0010311516411392091,0.00016004497789457115,0.00014875904632280287
0.10400000000000001,0.0010374821463344272,0.0001619318383345694,0.000150189829899245
0.10500000000000001,0.0010439906939353658,0.00016383317842627872,0.00015162118764055265
0.106,0.001050669589066362,0.0001657492674191068,0.0001530530981379013
0.107,0.0010575401052428089,0.00016768037757553287,0.00015448553956030778
0.108,0.001064594552970041,0.00016962678417989957,0.00015591848965009565
0.109,0.0010718349041941898,0.00017158876554712086,0.00015735192571823668
0.11,0.001079263135321181,0.0001735666030316572,0.0001587858246399136
0.111,0.001086881227222104,0.00017556058103588142,0.00016022016284952508
0.112,0.0010946925929932326,0.0001775709870194381,0.00016165491633653026
0.113,0.0011027024015492818,0.00017959811150744135,0.0001630900606402408
0.114,0.0011109076998102516,0.0001816422480998864,0.0001645255708456766
0.115,0.0011193104828802589,0.00018370369348002429,0.00016596142157845076
0.116,0.0011279031525008479,0.00018578274742361357,0.00016739758700040877
0.117,0.0011367069121350252,0.00018787971280731443,0.0001688340408045558
0.11800000000000001,0.0011457141688124527,0.00018999489561808002,0.00017027075621067487
0.11900000000000001,0.0011549269355896966,0.00019212860496152214,0.00017170770596022325
0.12000000000000001,0.001164347230023296,0.00019428115307131155,0.0001731448623119117
0.121,0.001173977074175203,0.0001964528553176488,0.0001745821970366096
0.122,0.0011838184946174077,0.00019864403021639928,0.00017601968141267831
0.123,0.001193873522436704,0.0002008549994381145,0.00017745728622127442
0.124,0.0012041441932399454,0.00020308608781667461,0.0001788949817412072
0.125,0.0012146325471585958,0.0002053376233585105,0.0001803327377443803
0.126,0.00122533106889122,0.00020760993725154608,0.00018177052349084962
0.127,0.0012362609314469932,0.00020990336387403735,0.0001832083077238317
0.128,0.001247414624728332,0.00021221824080353162,0.00018464605866482344
0.129,0.0012587942070144543,0.0002145549088262017,0.00018608374400892207
0.13,0.0012704017411339671,0.0002169137119454165,0.00018752133091953508
0.131,0.0012822392944695023,0.00021929499739105351,0.00018895878602366638
0.132,0.0012943089389626423,0.00022169911562847485,0.0001903960754069462
0.133,0.001306612751118901,0.00022412642036752318,0.0001918331646085422
0.134,0.0013191528120124806,0.00022657726857164306,0.0001932700186162652
0.135,0.001331931207291338,0.0002290520204668877,0.0001947066018614839
0.136,0.0013449405069364724,0.00023155103955110114,0.00019614287821416668
0.137,0.0013582018503225976,0.00023407469260281605,0.00019757881097771102
0.138,0.0013717078125475143,0.0002366233496905957,0.00019901436288404493
0.139,0.0013854604976028457,0.00023919738418208037,0.00020044949608848348
0.14,0.0013994620140784552,0.00024179717275297884,0.00020188417216455894
0.14100000000000001,0.0014137144751673076,0.00024442309539632307,0.00020331835209896218
0.14200000000000002,0.0014282199986702384,0.0002470755354317588,0.00020475199628656259
0.14300000000000002,0.0014429807070010991,0.0002497548795144054,0.00020618506452497692
0.14400000000000002,0.0014579987271914339,0.0002524615176442863,0.00020761757790907064
0.14500000000000002,0.001473276190895574,0.00025519584317537235,0.00020904946932497818
0.146,0.0014888124987927304,0.0002579582528249135,0.0002104806645074885
0.147,0.0015046229239468359,0.00026074914668234553,0.00021191112090306784
0.148,0.0015206996857316357,0.00026356892821907825,0.00021334079533664397
0.149,0.0015370449383141564,0.0002664180042970883,0.00021476964400584989
0.15,0.001553660840517462,0.00026929678517864165,0.00021619762247612948
0.151,0.0015705495558257312,0.0002722056845353621,0.000217624685675404
0.152,0.0015877132523892674,0.00027514511945747437,0.00021905078788863195
0.153,0.001605154103029225,0.0002781155104632109,0.00022047588275275396
0.154,0.0016228742852428732,0.0002811172815078673,0.00022189992325108706
0.155,0.001640875981208014,0.00028415085999344944,0.00022332286170830706
0.156,0.0016591519233801863,0.00028721667677770226,0.00022474464978484133
0.157,0.0016777232165898737,0.0002903151661836184,0.0002261652384716992
0.158,0.0016965825982383795,0.000293446766008671,0.00022758457808492744
0.159,0.001715732269276234,0.0002966119175342041,0.00022900261826030793
0.16,0.001735174435359449,0.00029981106553480884,0.00023041930794792152
0.161,0.0017549113068544436,0.00030304465828766595,0.000231834595406671
0.162,0.001774945098842949,0.000306313147582012,0.0002332484281989199
0.163,0.001795278031126985,0.00030961698872841026,0.00023466075318493137
0.164,0.0018159123282337438,0.0003129566405683047,0.00023607151651746036
0.165,0.001836850219420567,0.0003163325654833473,0.00023748066363619944
0.166,0.0018580845297372108,0.0003197452294048676,0.00023888813926229045
0.167,0.001879636320454557,0.00032319510182337154,0.0002402938873928316
0.168,0.0019014984214736506,0.0003266826557978326,0.00024169785129518045
0.169,0.0019236730810217452,0.00033020836796537894,0.00024309997350156133
0.17,0.0019461625520809246,0.0003337727185506151,0.0002445001958033505
0.171,0.0019689690923930725,0.00033737619137516085,0.0002458984592455212
0.17200000000000001,0.0019920949644646664,0.00034101927386724737,0.0002472947041210879
0.17300000000000001,0.0020155424355720046,0.00034470245707105457,0.00024868886996531723
0.17400000000000002,0.002039313777765782,0.00034842623565647425,0.00025008089555027436
0.17500000000000002,0.0020634112678762965,0.0003521911079284239,0.0002514707188789524
0.17600000000000002,0.0020878278259886074,0.0003559975758364579,0.0002528582771796419
0.177,0.0021125844664158506,0.00035984614498453917,0.0002542435069004144
0.178,0.0021376741139971372,0.0003637373246402979,0.0002556263437030815
0.179,0.002163112929586381,0.0003676716277448096,0.000257006722457652
0.18,0.002188900563587189,0.00037164957092220604,0.00025838457723660217
0.181,0.002215028736505574,0.00037567167448919914,0.00025975984130897434
0.182,0.002241499763190413,0.00037973846246473693,0.00026113244713464953
0.183,0.0022683159633190525,0.00038385046257967084,0.0002625023263585527
0.184,0.0022954796614022095,0.00038800820628642963,0.00026386940980485646
0.185,0.0023229931867891546,0.0003922122287684905,0.00026523362747094974
0.186,0.0023508495426739725,0.00039646306895033167,0.0002665949085218576
0.187,0.002379069735152282,0.00040076126950693545,0.0002679531812841659
0.188,0.0024076467720819212,0.00040510737687350705,0.00026930837324018887
0.189,0.0024365830022153507,0.00040950194125513866,0.00027066041102197794
0.19,0.002465880779168189,0.00041394551663666773,0.00027200922040552866
0.191,0.0024955424614241566,0.00041843866079236736,0.0002733547263048032
0.192,0.002525570412340266,0.00042298193529551357,0.0002746968527656004
0.193,0.0025559670001515915,0.0004275759055283402,0.00027603552295976896
0.194,0.002586734597976214,0.00043222114069180076,0.0002773706591791447
0.195,0.002617875583820346,0.00043691821381514913,0.0002787021828294437
0.196,0.002649383061072224,0.00044166770176594096,0.0002800300144243436
0.197,0.002681277981811149,0.00044647018525975445,0.00028135407357937663
0.198,0.00271355345398644,0.00045132624887001503,0.000282674279005886
0.199,0.002746211875206248,0.00045623648103777456,0.000283990779528406
0.2,0.002779296661528212,0.0004612014740815853,0.0002853037024033936
0.201,0.002812779856893036,0.0004662218242073377,0.0002866125399470723
0.202,0.002846654210480687,0.00047129813151821997,0.0002879172074802864
0.203,0.0028809221456425446,0.00047643100002440125,0.00028921761939215256
0.20400000000000001,0.002915586090672388,0.00048162103765297314,0.00029051368913399586
0.20500000000000002,0.00295064847881126,0.00048686885625806754,0.0002918053292133225
0.20600000000000002,0.0029861025047046405,0.0004921750716303784,0.00029309245118732877
0.20700000000000002,0.0030219691040814277,0.0004975403035074426,0.000294374965656978
0.20800000000000002,0.003058241476045338,0.0005029651755833086,0.0002956527822605615
0.20900000000000002,0.003094922073676763,0.0005084503155186225,0.00029692580966756045
0.21,0.0031320133550283217,0.000513996354950579,0.00029819395557237815
0.211,0.0031695177831299057,0.0005196039295027905,0.00029945712668800247
0.212,0.003207437825993652,0.0005252736787953409,0.0003007152287397217
0.213,0.0032457759566187987,0.0005310062464547975,0.0003019681664588722
0.214,0.0032845346529968454,0.0005368022801241474,0.0003032158435763996
0.215,0.00332371639811632,0.00054266243147289,0.00030445816281660424
0.216,0.003363314492175637,0.0005485873562069572,0.000305695025890676
0.217,0.0034033498094476838,0.0005545777140788928,0.00030692633349039503
0.218,0.0034438156544807025,0.0005606341688976937,0.0003081519852815766
0.219,0.003484714530301759,0.000566757388539049,0.00030937306167251035
0.22,0.00352604894495987,0.0005729480449554794,0.0003105883193738752
0.221,0.003567821411531315,0.0005792068141860952,0.00031179764233368927
0.222,0.0036100344481241734,0.0005855343763670799,0.00031300092644754034
0.223,0.003652690577883719,0.0005919314157415012,0.00031419806655662535
0.224,0.003695792328997106,0.0005983986206696312,0.00031538895644139375
0.225,0.0037393422346985723,0.0006049366836389247,0.00031657348881489737
0.226,0.00378333370333328,0.000611546301274298,0.00031775155531640827
0.227,0.003827787544027828,0.0006182281743481822,0.00031892304650472264
0.228,0.003872697169366137,0.0006249830077907337,0.0003200878518516918
0.229,0.003918065132820224,0.0006318115107000604,0.00032124585973562243
0.23,0.0039638939929341355,0.0006387143963522959,0.00032239695743461745
0.231,0.00401018631332877,0.0006456923822119088,0.0003235410311200055
0.232,0.004056944662706986,0.0006527461899418813,0.00032467879241809605
0.233,0.0041041716148585315,0.000659876545413893,0.0003258125172285007
0.234,0.0041518697486650335,0.0006670841787186909,0.0003269390600769445
0.23500000000000001,0.004200041648105094,0.0006743698241761087,0.00032805820423014885
0.23600000000000002,0.0042486808322936,0.0006817342203456205,0.00032916983144356556
0.23700000000000002,0.00429780804146436,0.0006891781100363723,0.00033027382233698633
0.23800000000000002,0.00434741679885708,0.0006967022403176156,0.00033137005638792243
0.23900000000000002,0.004397509708887914,0.0007043073625288874,0.0003324597394973729
0.24000000000000002,0.0044480893810948064,0.0007119942322904171,0.00033354163999663454
0.241,0.00449915843014255,0.0007197636095134513,0.0003346154480829152
0.242,0.004550719475827877,0.0007276162584104669,0.00033568170038733754
0.243,0.00460277514308435,0.000735552947505639,0.0003367401256828899
0.244,0.004655328061987329,0.000743574449645183,0.00033779145696983013
0.245,0.004708380867759087,0.0007516815420076874,0.00033883595996958945
0.246,0.004761927192936685,0.0007598750061144846,0.0003398734207849934
0.247,0.0048159877050575626,0.0007681556278400871,0.0003409021491829778
0.248,0.0048705560406670225,0.000776524197422522,0.00034192201493049454
0.249,0.0049256348556247515,0.0007849815094738773,0.00034293288659628847
0.25,0.004981226810962374,0.00079352836299059,0.00034393544825435726
0.251,0.005037334572888312,0.0008021655613639436,0.0003449301857866123
0.252,0.005093960812792939,0.0008108939123905403,0.0003459160112354587
0.253,0.005151108207253359,0.0008197142282827257,0.0003468923606980797
0.254,0.005208779438038742,0.000828627325679099,0.0003478590973545202
0.255,0.0052669771921148995,0.0008376340256550054,0.0003488160831517623
0.256,0.005325695218123014,0.0008467351537329474,0.0003497631787967866
0.257,0.005384954107043428,0.0008559315398932245,0.0003507002437497494
0.258,0.00544474761140609,0.0008652240185843613,0.00035162807816399696
0.259,0.005505078439014442,0.000874613428733684,0.00035254863098592876
0.26,0.005565949302894054,0.0008841006137578721,0.0003534597079188315
0.261,0.005627362921297234,0.0008936864215734912,0.00035436279191952246
0.262,0.0056893220177083766,0.0009033717046075754,0.0003552590425124948
0.263,0.005751829320848689,0.0009131573198081882,0.00035614524975957347
0.264,0.00581488756468147,0.0009230441286550725,0.0003570206505498013
0.265,0.005878499488416823,0.000933032997170202,0.0003578850970977173
0.266,0.005942658959511261,0.0009431247959284365,0.0003587384403336851
0.267,0.00600738648847001,0.0009533204000680838,0.0003595807680221883
0.268,0.006072675946516207,0.0009636206893016573,0.0003604194721894505
0.269,0.006138530093897969,0.0009740265479264183,0.0003612480602007724
0.27,0.006204951696135425,0.000984538864835098,0.0003620661170416931
0.271,0.006271943524025881,0.0009951585335265614,0.0003628758885850243
0.272,0.006339508353648513,0.001005886452116473,0.00036367488151205614
0.273,0.006407648966369693,0.0010167235233480671,0.0003644631146327697
0.274,0.00647636814884776,0.0010276706546027753,0.00036523932328024725
0.275,0.006545668693038297,0.001038728757910995,0.0003660033502493421
0.276,0.0066155445879547475,0.001049898749962838,0.0003667550370113074
0.277,0.006686016259650509,0.0010611815521188526,0.00036749422370681257
0.278,0.006757077700780559,0.0010725780904207634,0.0003682217076834328
0.279,0.006828731724539041,0.0010840892956023146,0.00036893808171171305
0.28,0.0069009811494420955,0.0010957161030999783,0.00036964421678644706
0.281,0.006973828799333264,0.001107459453063784,0.00037033952777131105
0.28200000000000003,0.007047277503388088,0.001119320290368092,0.00037102490026826767
0.28300000000000003,0.007121337496789484,0.0011312995646225795,0.0003716990858529527
0.28400000000000003,0.007196079082991386,0.0011433982301827903,0.00037236187655160136
0.28500000000000003,0.007271431287828912,0.0011556172461611566,0.0003730111262296115
0.28600000000000003,0.007347388211832858,0.001167957576437857,0.00037364764717651296
0.28700000000000003,0.007423970233572572,0.001180420189671621,0.0003742732258539113
0.28800000000000003,0.007501280616646572,0.001193006059310594,0.0003748848227076038
0.28900000000000003,0.007579229035790604,0.00120571616360336,0.00037548227845421076
0.29,0.007657803901144869,0.001218551485609711,0.0003760689998276283
0.291,0.0077370081019681285,0.0012315130132115068,0.00037664128262296386
0.292,0.007816844532920648,0.0012446017391237994,0.0003772057227905373
0.293,0.007897316094068976,0.0012578186609056516,0.0003777581080261455
0.294,0.007978425690891373,0.0012711647809710818,0.000378295692410518
0.295,0.008060176234282406,0.001284641106600044,0.0003788182977893195
0.296,0.008142561943019775,0.0012982486499494136,0.00037932574459472986
0.297,0.008225603141418751,0.001311988428063934,0.0003798183767565074
0.298,0.008309294051643391,0.0013258614628872485,0.0003802978873597981
0.299,0.008393637606304735,0.0013398687812729256,0.0003807725978150669
0.3,0.00847863674345569,0.0013540114149954148,0.00038123315485585175
0.301,0.00856429440659574,0.0013682904007611357,0.0003816798656512542
0.302,0.008650613544676295,0.0013827067802195002,0.00038211061766323085
0.303,0.008737597112105344,0.00139726159997398,0.0003825286642195939
0.304,0.008825248068752917,0.0014119559115931674,0.0003829331824915439
0.305,0.008913569379955777,0.0014267907716218342,0.00038332603897565926
0.306,0.009002555394994494,0.001441767241592078,0.00038370488964950913
0.307,0.009092226340941974,0.0014568863880343392,0.00038407702904967155
0.308,0.009182576570330524,0.001472149282488656,0.0003844342319518921
0.309,0.009273609070414919,0.0014875570015155874,0.0003847795115046943
0.31,0.009365326833941772,0.001503110626707586,0.0003851161600582799
0.311,0.00945773285915508,0.0015188112446999505,0.00038543710232743003
0.312,0.009550830149800784,0.0015346599471821006,0.0003857440173054738
0.313,0.00964462171513211,0.0015506578309087459,0.0003860364695839935
0.314,0.009739110569914401,0.0015668059977109957,0.00038631305269202387
0.315,0.009834299734430379,0.001583105554507667,0.00038657552650683233
0.316,0.009930183691336782,0.001599557613316404,0.0003868242339649728
0.317,0.010026782566231789,0.0016161632912649229,0.00038706372067245546
0.318,0.01012409084488642,0.001632923710602275,0.00038728999193320227
0.319,0.01022211156970289,0.0016498399987100855,0.00038750447954239526
0.32,0.01032084778862574,0.0016669132881137858,0.00038770488193987367
0.321,0.010420302555147188,0.0016841447164938936,0.0003879113435189903
0.322,0.010520478928311898,0.0017015354266972905,0.0003881181866509714
0.323,0.010621379972722172,0.0017190865667485555,0.0003883190768663706
0.324,0.01072300875854291,0.0017367992898612086,0.000388513516569228
0.325,0.010825368361506866,0.001754674754449064,0.00038869734548134494
0.326,0.010928453400551303,0.001772714124137567,0.00038887429797010913
0.327,0.011032283895506614,0.0017909185677750727,0.00038903781232117003
0.328,0.011136854468283927,0.0018092892594442909,0.0003891897669442162
0.329,0.011242168216937163,0.0018278273784735888,0.00038932805543788555
0.33,0.011348228245113152,0.0018465341094483793,0.0003894513547569949
0.331,0.011455037662056633,0.0018654106422225027,0.0003895637022278887
0.332,0.011562599582615473,0.0018844581719296583,0.0003896766317811301
0.333,0.011670917127245436,0.0019036778989947932,0.00038977906970542555
0.334,0.011779993422015717,0.0019230710291454824,0.00038987353055043854
0.335,0.011889831598613225,0.0019426387734234718,0.0003899521082775164
0.336,0.012000426415191463,0.001962382348196001,0.00039001690360868573
0.337,0.012111797781458999,0.001982302975167365,0.0003900673730355982
0.338,0.01222394045839952,0.00200240188139034,0.000390107527900177
0.339,0.012336857600223267,0.002022680299277653,0.00039013081389592064
0.34,0.012450552366784055,0.002043139466613476,0.000390139709644963
0.341,0.012565027923584047,0.0020637806265650003,0.0003901397516922013
0.342,0.012680287441779022,0.0020846050276938513,0.000390136305660907
0.343,0.012796334098183204,0.0021056139239677093,0.000390134154811279
0.34400000000000003,0.01291317107527458,0.0021268085747717376,0.00039013200711493745
0.34500000000000003,0.013030801561199686,0.002148190244920375,0.00039012315877727695
0.34600000000000003,0.013149220456294472,0.0021697602046685948,0.0003900992932157394
0.34700000000000003,0.013268447555730634,0.0021915197297236403,0.0003900653843492849
0.34800000000000003,0.013388477762527941,0.0022134701012566514,0.00039002107621133856
0.34900000000000003,0.013509314287558081,0.002235612605914179,0.0003899689277424378
0.35000000000000003,0.013630960347386877,0.002257948535829833,0.0003899201035795595
0.35100000000000003,0.013753419164279192,0.002280479188635912,0.0003898599618944029
0.35200000000000004,0.013876693966203725,0.002303205867475067,0.0003897850840413123
0.353,0.014000787986838509,0.0023261298810119094,0.00038969956969826683
0.354,0.01412570446557556,0.002349252543444588,0.0003896081663869518
0.355,0.014251446647526379,0.0023725751745166525,0.00038951792674794616
0.356,0.014378009578207293,0.0023960990995286232,0.0003894215910433245
0.357,0.014505412933776302,0.0024198256493496864,0.0003893303279293415
0.358,0.014633651762283945,0.0024437561604294484,0.0003892372104316738
0.359,0.014762729331769205,0.002467891974809569,0.00038913782027332367
0.36,0.014892648916015182,0.0024922344401355962,0.0003890441548979838
0.361,0.015023413794554855,0.0025167849096686323,0.00038893610756362954
0.362,0.01515502725267561,0.0025415447422971527,0.0003888283578110571
0.363,0.015287492581424705,0.0025665153025487024,0.0003887124936543787
0.364,0.015420813077613879,0.0025916979606017466,0.0003885922016222712
0.365,0.015554992043824906,0.00261709409229738,0.0003884929450269266
0.366,0.015690024673784757,0.0026427050791512094,0.0003883925713809848
0.367,0.01582593052009796,0.002668532308365156,0.0003882877504976745
0.368,0.015962704778872974,0.002694577172839199,0.0003881802858136963
0.369,0.016100350775821365,0.002720841071183319,0.00038809992314949325
0.37,0.0162388718424497,0.0027473254077292905,0.00038802627406194857
0.371,0.01637827131606468,0.0027740315925425464,0.00038796070106264665
0.372,0.016518552539778384,0.00280096104143408,0.0003878946921111832
0.373,0.01665971886251301,0.0028281151759722936,0.0003878386962858681
0.374,0.016801773639006222,0.0028554954234949297,0.0003878024122577811
0.375,0.016944720229815965,0.0028831032171209485,0.00038777644241312886
0.376,0.01708855397994138,0.002910939995762493,0.00038774383775898416
0.377,0.01723329431383154,0.0029390072041367357,0.00038770771586365876
0.378,0.01737893657871135,0.0029673062927779376,0.0003876787412332893
0.379,0.017525484158471015,0.0029958387180493195,0.00038764430467994683
0.38,0.017672940442846757,0.003024605942155059,0.00038760950781041267
0.381,0.017821308827425244,0.0030536094331522715,0.0003875895718036963
0.382,0.01797059271364926,0.0030828506649629938,0.00038760012947537155
0.383,0.018120795508822347,0.0031123311173862278,0.0003876186016706152
0.384,0.01827192062611413,0.0031420522761098735,0.00038765401376136425
0.385,0.018423971484565177,0.003172015632722823,0.0003876952497126601
0.386,0.018576943583540447,0.0032022226847269815,0.00038775665610277807
0.387,0.01873085621466841,0.0032326749355493156,0.0003878190530341308
0.388,0.018885704879380863,0.003263373894553939,0.0003879089031403354
0.389,0.019041493020253337,0.003294321077054121,0.00038805110671739354
0.39,0.019198224085757668,0.0033255180043244587,0.00038823695038168695
0.391,0.019355901530267308,0.0033569662036129332,0.0003884430304842831
0.392,0.0195145288140621,0.0033886672081529807,0.00038866017736237087
0.393,0.01967410940333358,0.0034206225571756974,0.0003888837252921136
0.394,0.019834646770189802,0.003452833795921912,0.0003891229301403145
0.395,0.019996144392660786,0.0034853024756543558,0.0003894033151855538
0.396,0.02015859792760272,0.003518030153669803,0.00038973392122235916
0.397,0.02032202652909514,0.0035510183933112715,0.00039009984728437133
0.398,0.020486425855899344,0.0035842687639801563,0.0003904913512196878
0.399,0.020651799409782835,0.003617782841148462,0.0003909223988738336
0.4,0.02081815069846007,0.0036515622063710037,0.0003913825476878213
0.401,0.020985483235597797,0.003685608447297585,0.00039189841510156684
0.402,0.021153800540819796,0.0037199231576852867,0.0003924609162270833
0.403,0.021323106139712365,0.0037545079374106793,0.0003930328640672182
0.404,0.02149340356382887,0.0037893643924820325,0.00039365711254123176
0.405,0.021664696350695355,0.0038244941350516507,0.000394319725110078
0.406,0.021836980317818135,0.0038598987834280933,0.00039501553143158496
0.40700000000000003,0.022010274476934728,0.003895579962088459,0.00039572390977367285
0.40800000000000003,0.022184574647291188,0.003931539301690822,0.00039647923989133155
0.40900000000000003,0.022359884390353926,0.003967778439086323,0.0003972933752881174
0.41000000000000003,0.022536207273587003,0.004004299017331642,0.00039813304137146957
0.41100000000000003,0.022713546870457495,0.004041102685701239,0.00039904327122279105
0.41200000000000003,0.0228919067604404,0.0040781910996998206,0.0003999961926032086
0.41300000000000003,0.023071290529023444,0.0041155659210745845,0.0004009730777933341
0.41400000000000003,0.023251701767712803,0.0041532288178276824,0.0004019833667830873
0.41500000000000004,0.023433144074037567,0.004191181464228462,0.0004030417884539525
0.41600000000000004,0.02361561342934494,0.0042294255408260465,0.00040419279800537483
0.41700000000000004,0.023799128698173518,0.004267962734461603,0.00040537664640089206
0.418,0.023983685863441767,0.0043067947382808645,0.00040658297765198373
0.419,0.024169288546822293,0.004345923251746316,0.00040781488592043206
0.42,0.024355940376036053,0.004385349980650015,0.0004090882279640792
0.421,0.024543644984857643,0.004425076637125757,0.00041044282412391176
0.422,0.02473240601312046,0.004465104939661649,0.00041186811670192766
0.423,0.02492222710672154,0.0045054366131125345,0.00041333263003387135
0.424,0.025113111917626645,0.0045460733887125555,0.00041485047283810605
0.425,0.025305064103875625,0.004587017004087577,0.0004163926304941369
0.426,0.025498079813880147,0.0046282692032677455,0.0004180090065128343
0.427,0.025692177760058006,0.004669831736699966,0.000419710003868596
0.428,0.025887354092220725,0.004711706361260521,0.00042147280168668263
0.429,0.026083612492754385,0.004753894840267507,0.00042332925402836145
0.43,0.026280956650144478,0.004796398943493495,0.0004252559414151181
0.431,0.026479390258980696,0.004839220447178041,0.0004272638959488171
0.432,0.026678917019962275,0.004882361134040259,0.00042935857988447086
0.433,0.026879540639903034,0.0049258227932914705,0.0004315932045141819
0.434,0.027081264831736163,0.004969607220647806,0.00043389693830078263
0.435,0.027284093314519836,0.0050137162183427186,0.00043628241627236973
0.436,0.027488022406986855,0.0050581515951397754,0.00043869742562347217
0.437,0.0276930706644472,0.0051029151663451585,0.00044115704549449735
0.438,0.027899234406858604,0.0051480087538203646,0.00044371032423134576
0.439,0.028106517377828658,0.005193434185994962,0.00044631499035262696
0.44,0.028314923327114837,0.0052391932978790865,0.0004489953727762965
0.441,0.028524456010629945,0.0052852879310762955,0.00045180030335113087
0.442,0.02873511919044684,0.005331719933796172,0.0004546931705425167
0.443,0.028946916634803824,0.005378491160867073,0.00045763865189486384
0.444,0.029159852118109456,0.0054256034737488685,0.0004606841033456741
0.445,0.02937392942094784,0.005473058740545578,0.00046383440767538693
0.446,0.029589145035663133,0.005520858836018291,0.0004670718941740309
0.447,0.02980551735540436,0.005569005641597786,0.00047041005781933937
0.448,0.030023042873562257,0.0056175010453973166,0.00047382987015673984
0.449,0.03024172539547383,0.005666346942225492,0.0004773679226452513
0.45,0.030461568732676733,0.005715545233598945,0.00048098518185797667
0.451,0.03068257670291441,0.005765097827755221,0.0004846592406235981
0.452,0.030904753130141644,0.005815006639665555,0.0004884427209367419
0.453,0.0311281018445292,0.005865273591047704,0.0004922998843943524
0.454,0.03135262668246887,0.005915900610378875,0.0004962219429454216
0.455,0.031578331486579084,0.005966889632908407,0.0005002202766675307
0.456,0.03180521292613823,0.006018242600670826,0.0005043147563627543
0.457,0.032033289227015795,0.006069961462498528,0.0005085453043265042
0.458,0.03226255705935549,0.00612204817403486,0.0005128979078666956
0.459,0.032493020290731596,0.006174504697746888,0.0005173250724623301
0.46,0.032724682794970116,0.006227333002938372,0.0005218353453110715
0.461,0.032957548452153665,0.006280535065762643,0.0005264771615655531
0.462,0.0331916211486269,0.006334112869235584,0.0005312580071924975
0.463,0.03342690477700116,0.006388068403248549,0.0005361457348068598
0.464,0.03366340323616018,0.006442403664581334,0.0005411427969207858
0.465,0.03390112043126445,0.006497120656915162,0.0005462307944362027
0.466,0.03414005321188376,0.0065522213908456185,0.0005514160696867882
0.467,0.03438021963142225,0.00660770788389569,0.0005567547265313284
0.468,0.03462161654013045,0.0066635821605288015,0.0005622037613504366
0.46900000000000003,0.034864247868328126,0.006719846252161658,0.0005677541459197181
0.47000000000000003,0.03510811755263817,0.00677650219717763,0.0005734379033767028
0.47100000000000003,0.03535322953599044,0.00683355204093935,0.0005792551818085723
0.47200000000000003,0.035599587767628026,0.006890997835802133,0.000585158170860326
0.47300000000000003,0.035847196203111345,0.006948841641126805,0.0005912104979327696
0.47400000000000003,0.03609605880432403,0.007007085523292892,0.0005974023981109286
0.47500000000000003,0.03634617953947771,0.007065731555711787,0.0006037004269143689
0.47600000000000003,0.03659755544182384,0.007124781818839605,0.0006101096486732046
0.47700000000000004,0.036850204387048814,0.007184238400190526,0.0006166178159393252
0.47800000000000004,0.03710412340889719,0.0072441033943497985,0.0006232279760509143
0.47900000000000004,0.03735931650094306,0.0073043789029869485,0.0006299726271076417
0.48000000000000004,0.037615787663114235,0.007365067034868847,0.0006368256973223724
0.481,0.03787354090169662,0.007426169905873029,0.0006437983807059457
0.482,0.03813258022934025,0.007487689639000496,0.0006508801571129679
0.483,0.038392909665063445,0.007549628364389396,0.0006580747060037751
0.484,0.038654533234258215,0.007611988219327867,0.0006653640366843027
0.485,0.03891745496869566,0.007674771348267334,0.0006727663893917122
0.486,0.039181672088733716,0.007737979902835802,0.0006802670643446546
0.487,0.03944720228702138,0.007801616041850983,0.0006878997183803303
0.488,0.03971404278421809,0.007865681931333583,0.0006956595460373859
0.489,0.03998219763766106,0.007930179744520543,0.0007035533719122228
0.49,0.04025167091109177,0.007995111661878324,0.0007115381847504486
0.491,0.04052246667466106,0.008060479871116168,0.0007196660973496781
0.492,0.04079458900493439,0.00812628656719938,0.0007279565435563254
0.493,0.04106804198489654,0.008192533952362654,0.0007363762549268953
0.494,0.04134282970395699,0.008259224236123366,0.0007449028304237237
0.495,0.04161895625795512,0.008326359635294885,0.0007535528067077336
0.496,0.04189641905781389,0.008393942373999937,0.0007623159274183798
0.497,0.042175235607757225,0.008461974683683897,0.0007711763132637034
0.498,0.04245540331881504,0.008530458803128258,0.0007801487027502963
0.499,0.04273692631259611,0.008599396978463878,0.0007892903020437007
0.5,0.04301980871716492,0.00866879146318443,0.0007985383191788098
0.501,0.04330405466704573,0.008738644518159793,0.0008079687943351177
0.502,0.04358966830322833,0.00880895841164945,0.0008175488487372396
0.503,0.04387665377317321,0.008879735419315821,0.0008273303071973489
0.504,0.04416501523081593,0.008950977824237882,0.0008372766879825766
0.505,0.04445475683657301,0.009022687916924501,0.0008473829546234788
0.506,0.04474587619542574,0.00909486799532777,0.0008576479959616094
0.507,0.04503839061771705,0.009167520364856688,0.000868067026154364
0.508,0.04533229770833659,0.009240647338390475,0.0008786594583326555
0.509,0.04562760165367444,0.00931425123629216,0.0008894458753939384
0.51,0.04592430664662634,0.00938833438642204,0.0009003693972519715
0.511,0.04622241688659927,0.009462899124151105,0.0009114458843359227
0.512,0.04652193657951685,0.009537947792374766,0.0009226205593359176
0.513,0.04682286993782339,0.009613482741526206,0.0009339297923880438
0.514,0.04712522118049012,0.00968950632959001,0.0009453672801664895
0.515,0.04742899453301985,0.009766020922115622,0.0009569214767992184
0.516,0.0477341877979796,0.009843028892231143,0.0009686542998793609
0.517,0.04804081808630664,0.009920532620656662,0.0009805420183019897
0.518,0.04834888320027519,0.009998534495717946,0.0009926018837997195
0.519,0.048658387391564834,0.01007703691336012,0.0010048183724906963
0.52,0.04896933491841224,0.01015604227716109,0.0010171583448234912
0.521,0.049281730045616416,0.010235552998345481,0.0010296146285921413
0.522,0.049595577044543177,0.010315571495797898,0.0010421983864659858
0.523,0.049910880193130745,0.010396100196076919,0.0010549910296013933
0.524,0.05022764377589483,0.010477141533428509,0.001067923623046552
0.525,0.05054587208393333,0.010558697949799824,0.0010809955547354806
0.526,0.05086556312096206,0.010640771894852904,0.0010942184482312775
0.527,0.051186733792918625,0.010723365825978297,0.0011075803169808965
0.528,0.05150938210302038,0.010806482208308833,0.0011210802666797978
0.529,0.05183351236874624,0.010890123514733303,0.0011347305451765567
0.53,0.05215912891418298,0.010974292225910225,0.001148566928710055
0.531,0.052486236070030425,0.011058990830281534,0.0011625426651508282
0.532,0.05281483817360636,0.01114422182408642,0.0011766462123520938
0.533,0.05314493956885189,0.011229987711375069,0.0011908976428115475
0.534,0.05347654460633658,0.011316291004022417,0.00120530134762859
0.535,0.05380965764326303,0.011403134221741896,0.0012198604851110955
0.536,0.0541442768880925,0.011490519892099411,0.0012345838335143453
0.537,0.054480419036100146,0.01157845055052693,0.001249468001044737
0.538,0.05481808229504048,0.011666928740336455,0.0012645212932280245
0.539,0.05515727104870085,0.011755957012733905,0.0012797112515630159
0.54,0.055497989687527435,0.011845537926832801,0.001295096167218965
0.541,0.05584024260863047,0.011935674049668195,0.0013106961409978185
0.542,0.056184034215788964,0.01202636795621062,0.0013264590616574143
0.543,0.05652936891945642,0.012117622229379975,0.0013423901661339872
0.544,0.056876251136765185,0.0122094394600592,0.0013584595129836688
0.545,0.05722468529153249,0.012301822247108534,0.0013746748436173147
0.546,0.057574669800597424,0.012394773197379156,0.0013910983126718865
0.547,0.05792622114283945,0.012488294925727186,0.0014076825949276082
0.548,0.05827933773417912,0.012582390055027707,0.0014244099950414771
0.549,0.0586340240252218,0.012677061216188692,0.00144127753559759
0.55,0.05899028447328255,0.012772311048164892,0.0014583191285525102
0.551,0.059348123542391315,0.012868142197971912,0.0014755253657967925
0.552,0.059707545703298094,0.012964557320700119,0.0014929208175250555
0.553,0.06006855543347782,0.01306155907952879,0.001510482044903877
0.554,0.06043115721713578,0.013159150145739837,0.0015282338722259958
0.555,0.060795355545212676,0.013257333198732207,0.0015461554792426829
0.556,0.06116114904659356,0.01335611092603562,0.0015642372769754864
0.557,0.061528553977958485,0.013455486023324739,0.0015824844975218186
0.558,0.06189756896705863,0.01355546119443327,0.0016008890306859304
0.559,0.062268198531826885,0.013656039151367901,0.0016194841579464437
0.56,0.06264044719695637,0.013757222614322552,0.0016382375364213868
0.561,0.06301431949390662,0.013859014311692319,0.0016571822682443981
0.562,0.06338981996090784,0.013961416980087677,0.0016763149479678246
0.5630000000000001,0.0637669531429665,0.014064433364348464,0.0016956093859516051
0.5640000000000001,0.0641457235918702,0.014168066217558417,0.0017150669705743708
0.5650000000000001,0.06452613586619245,0.014272318301058753,0.0017347288323097752
0.5660000000000001,0.06490818881056776,0.014377192384462577,0.0017546129177616987
0.5670000000000001,0.06529189845360293,0.014482691245669177,0.0017746877578608598
0.5680000000000001,0.06567726363857897,0.014588817670877963,0.001794954623906408
0.5690000000000001,0.06606428895126562,0.01469557445460286,0.0018154342205038275
0.5700000000000001,0.06645297898424465,0.014802964399686386,0.001836164859407928
0.5710000000000001,0.06684333833691404,0.014910990317313865,0.001857077439757595
0.5720000000000001,0.06723537161549455,0.015019655027027705,0.0018781626778627569
0.5730000000000001,0.06762908343303324,0.015128961356741634,0.0018994619509131224
0.5740000000000001,0.06802447840940945,0.015238912142754888,0.001920932419500941
0.5750000000000001,0.06842156117134006,0.015349510229766501,0.0019425868326728186
0.5760000000000001,0.06882033078294751,0.01546075847088965,0.0019644702227071234
0.5770000000000001,0.06922080303881967,0.015572659727665679,0.0019865515793827783
0.578,0.06962297700150308,0.015685216870078903,0.0020088092333154233
0.579,0.0700268573251147,0.015798432776570143,0.0020312874146293613
0.58,0.0704324486706333,0.01591231033405183,0.0020539561843914214
0.581,0.0708397557059065,0.01602685243792189,0.0020768166932944422
0.582,0.07124878310565391,0.016142061992078134,0.0020999232905168546
0.583,0.07165953555147382,0.01625794190893275,0.002123244014706802
0.584,0.07207201773184709,0.016374495109426516,0.0021467515620533827
0.585,0.07248623434214319,0.016491724523043275,0.002170481547534356
0.586,0.0729021846697477,0.01660963308782414,0.0021944186331609096
0.587,0.07331988426921228,0.01672822375038226,0.0022185713002128953
0.588,0.07373933242612106,0.016847499465916807,0.0022429498663292706
0.589,0.07416053386344687,0.0169674631982277,0.0022675257183384506
0.59,0.07458349331107643,0.01708811791972986,0.0022923157939983676
0.591,0.07500821550581559,0.01720946661146779,0.002317419483751931
0.592,0.07543470519139375,0.01733151226312991,0.0023427309300565547
0.593,0.07586296711846904,0.017454257873063025,0.0023682396486550514
0.594,0.07629300604463457,0.017577706448287028,0.0023939468072749766
0.595,0.07672482673442184,0.017701861004509142,0.0024198622598074855
0.596,0.07715842870229038,0.017826724566138354,0.0024459945575429094
0.597,0.0775938272566676,0.01795230016630029,0.0024723453688009055
0.598,0.07803102190998103,0.018078590846851414,0.002498906788067602
0.599,0.07847001745457022,0.018205599658393717,0.0025256808794151776
0.6,0.07891081868973972,0.01833332966028923,0.0025526796047271416
0.601,0.07935343042176292,0.018461783920674484,0.002579885821718908
0.602,0.079797857463889,0.018590965516475298,0.0026073126100028044
0.603,0.08024410463634661,0.018720877533421252,0.002634963210593714
0.604,0.08069217676634956,0.01885152306606016,0.0026628252079338435
0.605,0.08114207868810182,0.018982905217772877,0.002690917305521481
0.606,0.08159381014698516,0.019115027100787815,0.0027193247137385734
0.607,0.0820473861991392,0.019247891836195574,0.0027479807930473085
0.608,0.08250280658768043,0.01938150255396366,0.002776878215434041
0.609,0.08296007617482438,0.019515862392950934,0.002805997338200224
0.61,0.08341919982980281,0.019650974500922548,0.002835386600136836
0.611,0.08388018242886724,0.019786842034564482,0.0028650230376726683
0.612,0.08434302885529632,0.0199234681594982,0.002894907158371188
0.613,0.0848077439993986,0.020060856050295395,0.0029250165747441853
0.614,0.0852743327585192,0.020199008890492712,0.002955352582457667
0.615,0.08574280003704414,0.020337929872606495,0.0029859489251914863
0.616,0.0862131458151611,0.020477622198147395,0.0030167836685293372
0.617,0.08668538489048769,0.020618089077635304,0.0030478492991459103
0.618,0.08715951724070957,0.020759333730613918,0.0030791471372799135
0.619,0.0876355477984284,0.02090135938566568,0.0031106785088079424
0.62,0.0881134815033122,0.02104416928042638,0.0031424447452611777
0.621,0.08859332330210211,0.021187766661600185,0.003174447183841755
0.622,0.08907507814861444,0.021332154784974185,0.0032067195753841637
0.623,0.08955875100374837,0.02147733691543339,0.0032392374291899608
0.624,0.09004434683549037,0.02162331632697547,0.0032719958900108374
0.625,0.09053187061891817,0.021770096302725705,0.0033049963200288126
0.626,0.09102132257294596,0.021917680134951566,0.0033382770339944043
0.627,0.09151271723036217,0.022066071125077913,0.00337180754473739
0.628,0.09200605480733776,0.022215272583701713,0.003405584527238577
0.629,0.09250134030737063,0.02236528783060681,0.0034396349135252554
0.63,0.09299857874107577,0.022516120194779075,0.003473937690446738
0.631,0.09349777512619205,0.022667773014421036,0.0035084913857634527
0.632,0.09399893448758563,0.02282024963696714,0.0035432974062503055
0.633,0.09450206185725527,0.022973553419098267,0.003578357164581716
0.634,0.09500716227433821,0.02312768772675698,0.0036136720793486636
0.635,0.09551424078511479,0.023282655935162468,0.0036493434600416113
0.636,0.09602329785118256,0.023438461428825212,0.0036853096708195066
0.637,0.09653434773411954,0.02359510760156244,0.0037216243028802137
0.638,0.0970473908925355,0.023752597856512694,0.003758217294947416
0.639,0.0975624324013346,0.023910935606151033,0.0037950814968893435
0.64,0.09807947734258962,0.024070124272303976,0.0038322755754688505
0.641,0.09859853080554652,0.024230167286164596,0.003869737928077895
0.642,0.09911959788663077,0.024391068088307537,0.003907485334266426
0.643,0.09964268368945113,0.02455283012870393,0.003945527914856953
0.644,0.10016779332480598,0.024715456866736644,0.0039838433342789855
0.645,0.10069493191068749,0.024878951771215324,0.00402246335297859
0.646,0.10122410015537212,0.025043318320391195,0.004061364516286227
0.647,0.10175531204277057,0.025208560001972663,0.004100543366213941
0.648,0.10228856827792392,0.025374680313139848,0.004140001425695905
0.649,0.10282387400765194,0.02554168276056028,0.004179740223922898
0.65,0.10336123438599377,0.025709570860403496,0.0042197755618235445
0.651,0.10390065457421428,0.02587834813835654,0.0042601245995577165
0.652,0.10444213974080747,0.026048018129638764,0.004300759394558034
0.653,0.10498569506150258,0.026218584379017612,0.004341681503480503
0.654,0.1055313257192685,0.026390050440823053,0.0043828937685991215
0.655,0.10607903690431912,0.026562419878963264,0.004424427289730358
0.656,0.10662882957564247,0.02673569626693956,0.004466253108481655
0.657,0.10718071743295177,0.02690988318786183,0.00450837280865176
0.658,0.10773470143174622,0.027084984234463632,0.004550787980474163
0.659,0.10829078679127237,0.02726100300911719,0.004593500220635207
0.66,0.10884897873804632,0.02743794312384928,0.004636511132292192
0.661,0.10940928250586057,0.027615808200355783,0.004679822325091551
0.662,0.10997170333578837,0.02779460187001723,0.004723464788579645
0.663,0.11053624647618843,0.02797432777391432,0.004767453910605057
0.664,0.11110291718271091,0.02815498956284283,0.004811769452058971
0.665,0.11167172071830243,0.02833659089732897,0.004856405126790197
0.666,0.11224265829673034,0.02851913544764507,0.004901365246079844
0.667,0.1128157433269054,0.02870262689382441,0.004946636519414195
0.668,0.11339097701885181,0.02888706892567678,0.004992220608507968
0.669,0.11396836466475192,0.02907246524280397,0.005038119181737784
0.67,0.11454791156410896,0.02925881955461479,0.00508433391416063
0.671,0.11512962302375311,0.02944613558034074,0.005130866487532419
0.672,0.11571350435784669,0.02963441704905126,0.005177718590326552
0.673,0.11629956088788869,0.029823667699669067,0.005224891917752519
0.674,0.11688779794271972,0.03001389128098566,0.005272388171774627
0.675,0.11747822085852892,0.03020509155167683,0.005320209061130481
0.676,0.11807083110797077,0.030397272280317772,0.005368356301349975
0.677,0.11866564180247284,0.03059043724539871,0.005416831614773647
0.678,0.11926265441068767,0.03078459023534053,0.005465636730571796
0.679,0.11986187429824281,0.030979735048509902,0.005514773384763074
0.68,0.12046330683813923,0.031175875493234986,0.005564243320233356
0.681,0.12106695741075485,0.03137301538782076,0.005614048286754616
0.682,0.12167283140385093,0.03157115856056466,0.005664190041003825
0.683,0.12228093421257613,0.031770308849771944,0.005714670346581851
0.684,0.12289127123947284,0.03197047010377138,0.005765490974032355
0.685,0.12350384789448123,0.03217164618093074,0.0058166537008608795
0.686,0.12411866591328925,0.03237384094967206,0.0058681603115538225
0.687,0.12473573810308394,0.03257705828848754,0.005920012597597442
0.6880000000000001,0.12535506619528755,0.032781302085954915,0.005972212357497092
0.6890000000000001,0.12597665562948376,0.03298657624075341,0.006024764044491282
0.6900000000000001,0.12660051185267973,0.03319288466167862,0.006077743228191508
0.6910000000000001,0.1272266403193124,0.03340023126765866,0.006131075982806441
0.6920000000000001,0.12785504649125135,0.03360861998776964,0.006184764138628145
0.6930000000000001,0.12848573583780537,0.033818054761251305,0.006238809533077458
0.6940000000000001,0.12911871383572762,0.03402853953752252,0.0062932140107233294
0.6950000000000001,0.12975398596922028,0.034240078276197086,0.006347979423302014
0.6960000000000001,0.13039155424118729,0.03445267494709938,0.0064031313683910705
0.6970000000000001,0.13103143114774285,0.03466633353027992,0.006458709356591371
0.6980000000000001,0.13167361868725835,0.03488105801603104,0.006514654578893355
0.6990000000000001,0.13231812237378296,0.0350968524049028,0.006570968919589422
0.7000000000000001,0.1329649477288416,0.03531372070771849,0.006627654270250965
0.7010000000000001,0.1336141002814381,0.0355316669455903,0.006684712529747992
0.7020000000000001,0.13426558556806137,0.03575069514993506,0.006742171264058859
0.7030000000000001,0.13491940913269035,0.03597080936249027,0.006800071446881086
0.7040000000000001,0.13557557652679858,0.03619201363532957,0.006858351017530896
0.705,0.13623409330936032,0.03641431203087848,0.006917011908127565
0.706,0.13689496175471746,0.03663770862193009,0.0069760560582025405
0.707,0.13755819404100147,0.03686220749166123,0.007035485414718632
0.708,0.1382237924377506,0.03708781273364801,0.007095301932090161
0.709,0.13889176253399002,0.037314528451881525,0.007155507572202841
0.71,0.13956210992627088,0.037542358760783816,0.007216104304433593
0.711,0.14023484021867516,0.03777130778522386,0.007277094105670453
0.712,0.1409099590228211,0.038001379660532936,0.007338478960332658
0.713,0.14158747195786692,0.03823257853252103,0.007400260860390512
0.714,0.1422673846505175,0.03846490855749215,0.007462441805385482
0.715,0.14294970273502833,0.03869837390226065,0.007525023802450171
0.716,0.14363442876143956,0.03893297874416691,0.007588008866328556
0.717,0.14432157458291325,0.03916872727109326,0.007651462193480327
0.718,0.1450111427444102,0.03940562368147993,0.007715441060981379
0.719,0.14570313891044234,0.03964367218434079,0.007779830474142846
0.72,0.14639756875309695,0.0398828769992796,0.007844650896037473
0.721,0.14709443795204433,0.040123242356505634,0.00790996033883186
0.722,0.14779375219454097,0.040364772496849964,0.007975687254872398
0.723,0.14849551717543477,0.040607471671780984,0.00804183372328186
0.724,0.1491997385971713,0.04085134414342089,0.008108401830993206
0.725,0.14990642216979824,0.0410963941845613,0.00817539367277009
0.726,0.15061557072335233,0.04134262607867895,0.008242811351227322
0.727,0.15132719577896134,0.041590044119952936,0.00831065697685143
0.728,0.1520413001613057,0.041838652613279494,0.008378932668021184
0.729,0.15275788961089157,0.042088455874288264,0.008447640551028191
0.73,0.1534769698758545,0.04233945822935885,0.008516782760097645
0.731,0.15419854671196015,0.04259166401563645,0.008586361437408799
0.732,0.15492262588261504,0.042845077581048115,0.008656421286547818
0.733,0.15564921315886662,0.043099703284318454,0.008726972249446836
0.734,0.15637831431941113,0.04335554549498649,0.008797966896107155
0.735,0.1571099351505972,0.0436126085934208,0.008869407404540808
0.736,0.15784407876679657,0.04387089697083657,0.008941295960832346
0.737,0.15858075634996144,0.04413041502931079,0.009013634759159807
0.738,0.15931997100882395,0.044391167181799175,0.009086426001815669
0.739,0.1600617285603962,0.044653157852152195,0.009159671899227718
0.74,0.16080603482936892,0.044916391475130324,0.009233374669980147
0.741,0.16155289564811715,0.045180872496421845,0.009307536540834587
0.742,0.16230231685670463,0.045446605372657344,0.00938215974675103
0.743,0.1630543043028886,0.045713594571427145,0.00945725318861507
0.744,0.16380886384212537,0.04598184457129696,0.009532869619608923
0.745,0.16456600133757512,0.04625135986182379,0.009608954653687675
0.746,0.1653257201923217,0.046522144943573256,0.009685510561518533
0.747,0.1660880312419202,0.046794204328134664,0.009762539622083854
0.748,0.16685293788352837,0.047067542538137684,0.00984004412270241
0.749,0.16762044601117257,0.047342164107268846,0.009918026359050822
0.75,0.16839056152661128,0.04761807358028753,0.009996488635184824
0.751,0.1691632903393364,0.0478952755130425,0.010075433263560692
0.752,0.1699386383665792,0.04817377447248761,0.010154862565056686
0.753,0.17071661153331627,0.04845357503669899,0.010234778868994474
0.754,0.1714972157722745,0.04873468179489083,0.010315184513160687
0.755,0.17228045702393532,0.049017099347431474,0.010396081843828436
0.756,0.17306633898450957,0.04930083230586055,0.010477473215778792
0.757,0.17385487213585768,0.04958588529290452,0.010559360992322554
0.758,0.17464606016797393,0.04987226294249339,0.010641747545321682
0.759,0.17543990905241105,0.05015996989977721,0.010724635255211166
0.76,0.17623642476850224,0.05044901082114218,0.010808026511020523
0.761,0.17703561330336615,0.05073939037422738,0.010891923710395665
0.762,0.17783748065191307,0.0510311132379407,0.010976329259620644
0.763,0.17864203281684798,0.05132418410247594,0.011061245573639399
0.764,0.1794492758086782,0.05161860766932849,0.011146675076077672
0.765,0.18025921564571476,0.051914388651312135,0.011232620199264751
0.766,0.18107185632175343,0.05221153177257587,0.011319129825865875
0.767,0.18188720795757995,0.05251004176861954,0.0114061730550749
0.768,0.18270527454047764,0.052809923386311165,0.011493739724660888
0.769,0.18352606212003397,0.053111181383902854,0.011581832304433997
0.77,0.18434957675366812,0.05341382053104745,0.011670453273027773
0.771,0.18517582450663603,0.05371784560881529,0.011759660357712897
0.772,0.1860048114520342,0.05402326140971014,0.011849439407783933
0.773,0.1868365436708065,0.05433007273768678,0.01193975505673279
0.774,0.1876710272517502,0.05463828440816608,0.012030609822313814
0.775,0.1885082682915174,0.05494790124805292,0.012122034856393437
0.776,0.1893482710859818,0.05525892809575195,0.012214097122915856
0.777,0.19019104538739764,0.05557136980118454,0.012306707029638224
0.778,0.19103659548482915,0.05588523122580517,0.012399867134693366
0.779,0.1918849275064071,0.05620051724261806,0.012493580005267598
0.78,0.19273604758814683,0.056517232736193926,0.012587848217623173
0.781,0.19358996187395033,0.05683538260268655,0.012682674357120987
0.782,0.19444667651561182,0.05715497174984941,0.012778061018242994
0.783,0.19530619767282287,0.0574760050970518,0.01287401080461466
0.784,0.1961685315131793,0.057798487575296785,0.01297052632902797
0.785,0.19703368421218398,0.058122424127236366,0.013067610213463723
0.786,0.19790166037232582,0.058447819707189354,0.013165265089114449
0.787,0.19877246936978715,0.058774679281157205,0.013263493596406998
0.788,0.19964611579994496,0.05910300782684143,0.013362298385025393
0.789,0.20052260586998572,0.059432810333659616,0.013461682113933659
0.79,0.20140194579502682,0.05976409180276283,0.013561771221934015
0.791,0.20228414179812715,0.0600968572470518,0.013662459083493431
0.792,0.2031692001102878,0.06043111169119399,0.013763734941625772
0.793,0.20405712697045833,0.06076686017164022,0.013865601497537976
0.794,0.20494792862554279,0.061104107736641634,0.0139680614618488
0.795,0.20584161133040366,0.06144285944626619,0.014071117554611904
0.796,0.2067381799987207,0.06178312037241552,0.014174772505338933
0.797,0.20763764362298623,0.0621248955988422,0.014279029053022672
0.798,0.20854000710946208,0.06246819022116573,0.014383889946160171
0.799,0.2094452767448956,0.06281300934688995,0.014489357942775869
0.8,0.21035345882402243,0.06315935809541993,0.014595435810444842
0.801,0.21126455964956323,0.06350724159807844,0.014702185371735267
0.802,0.2121785855322373,0.06385666499812301,0.014809567320519041
0.803,0.21309554279076104,0.06420763345076301,0.014917568077363
0.804,0.2140154377518557,0.06456015212317603,0.015026190451165891
0.805,0.2149382767502542,0.06491422619452537,0.015135437260504965
0.806,0.21586406501544128,0.06526986085597626,0.015245311333659393
0.807,0.2167928111485208,0.06562706131071351,0.015355815508633904
0.808,0.2177245203712502,0.06598583277395799,0.015466952633182098
0.809,0.218659199050451,0.06634618047298359,0.015578725564830254
0.81,0.21959685356098035,0.06670810964713461,0.015691137170900732
0.811,0.22053749028573535,0.06707162554784178,0.015804190328535715
0.812,0.22148111561566036,0.06743673343864023,0.01591788792472089
0.8130000000000001,0.2224277359497472,0.06780343859518598,0.01603223285630921
0.8140000000000001,0.22337735769504646,0.06817174630527335,0.016147228030044366
0.8150000000000001,0.22432998726666778,0.06854166186885101,0.01626287636258491
0.8160000000000001,0.22528563021456016,0.06891319059804021,0.01637918078052788
0.8170000000000001,0.22624429474065735,0.06928633781715068,0.016496144220432753
0.8180000000000001,0.22720598638686462,0.06966110886269902,0.016613769628845185
0.8190000000000001,0.22817071160058444,0.07003750908342421,0.016732059962321067
0.8200000000000001,0.22913847683730842,0.07041554384030582,0.01685101818745047
0.8210000000000001,0.23010928856061827,0.0707952185065808,0.01697064728088147
0.8220000000000001,0.231083153242191,0.07117653846776002,0.01709095022934442
0.8230000000000001,0.23206007736180706,0.0715595091216461,0.01721193002967594
0.8240000000000001,0.233040067407352,0.07194413587835052,0.017333589688842785
0.8250000000000001,0.2340231298748229,0.07233042416030977,0.017455932223966325
0.8260000000000001,0.23500927063932966,0.07271837940230402,0.017578960662346498
0.8270000000000001,0.235998497495773,0.07310800705147275,0.017702678041486043
0.8280000000000001,0.2369908163109,0.07349931256733248,0.01782708740911483
0.8290000000000001,0.23798623361320517,0.07389230142179497,0.017952191823214003
0.8300000000000001,0.2389847559393212,0.07428697909918223,0.018077994352040373
0.8310000000000001,0.23998638983402204,0.07468335109624591,0.018204498074150796
0.8320000000000001,0.24099114185023165,0.07508142292218288,0.01833170607842645
0.8330000000000001,0.24199901854902342,0.07548120009865349,0.01845962146409732
0.834,0.24301002649962844,0.07588268815979832,0.018588247340766473
0.835,0.244024172279443,0.07628589265225524,0.01871772876076784
0.836,0.24504146209347288,0.07669081913517693,0.018848117756123228
0.837,0.24606190332164332,0.07709747318024875,0.01897922883656568
0.838,0.24708550216027586,0.07750586037170425,0.019111065162459282
0.839,0.24811226521946503,0.07791598630634443,0.01924362990468963
0.84,0.24914219911749647,0.07832785659355372,0.01937692624468862
0.841,0.2501753104808459,0.07874147685531825,0.019510957374459334
0.842,0.2512116059441889,0.07915685272624186,0.01964572649660061
0.843,0.25225109215040425,0.07957398985356506,0.019781236824332138
0.844,0.25329377575057876,0.07999289389718062,0.019917491581519085
0.845,0.25433966340401404,0.08041357052965238,0.020054494002696977
0.846,0.2553887616503935,0.08083602543623165,0.020192247333096738
0.847,0.256441077446637,0.08126026431487579,0.02033075482866964
0.848,0.2574966173234175,0.08168629287626343,0.020470019756112203
0.849,0.2585553879729395,0.08211411684381437,0.020610045392891362
0.85,0.25961739609564777,0.08254374195370506,0.020750835027269394
0.851,0.26068264840023075,0.08297517395488724,0.020892391958328968
0.852,0.2617511516036256,0.08340841860910433,0.021034719495998694
0.853,0.26282291243102435,0.08384348169091009,0.021177820961077676
0.854,0.2638979376158782,0.08428036898768465,0.021321699685261337
0.855,0.26497623389990244,0.08471908629965343,0.021466359011166065
0.856,0.26605780816227853,0.08515963943990353,0.021611802292355084
0.857,0.26714266692881417,0.08560203423440138,0.021758032893363456
0.858,0.2682308170693477,0.0860462765220106,0.021905054189723293
0.859,0.2693222653587016,0.08649237215450946,0.02205286956798949
0.86,0.2704170185799906,0.08694032699660834,0.02220148242576495
0.861,0.27151508352462356,0.08739014692596643,0.02235089617172605
0.862,0.27261646699230846,0.08784183783321108,0.022501114225648336
0.863,0.2737211757910593,0.08829540562195357,0.02265214001843171
0.864,0.2748292167372005,0.08875085620880721,0.02280397699212628
0.865,0.27594059665537113,0.08920819552340599,0.022956628599957965
0.866,0.27705532276911393,0.08966742950842035,0.023110098306353976
0.867,0.2781734011649263,0.09012856411957582,0.02326438958696858
0.868,0.2792948390566716,0.09059160532567122,0.023419505928708922
0.869,0.2804196433023016,0.09105655910859434,0.023575450829760484
0.87,0.281547820768108,0.09152343146334176,0.023732227799613304
0.871,0.2826793783287296,0.09199222839803477,0.023889840359087467
0.872,0.28381432286715325,0.09246295593393841,0.02404829204035901
0.873,0.2849526612747244,0.09293562010547794,0.024207586386986026
0.874,0.2860944004511479,0.0934102269602569,0.024367726953934306
0.875,0.2872395473044971,0.09388678255907565,0.024528717307603618
0.876,0.2883881094075781,0.09436529297594752,0.024690561025853437
0.877,0.28954009239930356,0.09484576429811778,0.024853261698029233
0.878,0.29069550384246007,0.09532820262608095,0.02501682292498837
0.879,0.2918543506786364,0.09581261407359816,0.02518124831912629
0.88,0.29301663985781123,0.09629900476771498,0.025346541504402714
0.881,0.2941823783383606,0.09678738084878034,0.02551270611636778
0.882,0.29535157308705995,0.0972777484704625,0.02567974580218833
0.883,0.2965242310790944,0.09777011379976792,0.02584766422067407
0.884,0.29770035929806016,0.09826448301705867,0.026016465042304017
0.885,0.29887996473596945,0.09876086231607041,0.02618615194925257
0.886,0.3000630553198401,0.09925925790393025,0.026356728635416472
0.887,0.3012496362326377,0.09975967600117458,0.026528198806440407
0.888,0.3024397153910147,0.1002621228417663,0.026700566179744076
0.889,0.30363329982070475,0.10076660467311312,0.0268738344845485
0.89,0.30483039655588184,0.10127312775608599,0.027048007461902435
0.891,0.3060310126391668,0.1017816983650358,0.02722308886470905
0.892,0.3072351551216355,0.10229232278781203,0.027399082457752577
0.893,0.308442831062818,0.1028050073257804,0.027575992017724756
0.894,0.3096540475307103,0.10331975829384064,0.027753821333251664
0.895,0.310868811601776,0.1038365820204453,0.027932574204920412
0.896,0.31208713156222884,0.10435548484761568,0.02811225444530584
0.897,0.31330901213064194,0.10487647313096192,0.028292865878997236
0.898,0.3145344615825186,0.10539955323969959,0.02847441234262529
0.899,0.3157634870282434,0.10592473155666854,0.02865689768488901
0.9,0.31699609558669545,0.10645201447834976,0.02884032576658223
0.901,0.3182322943852511,0.10698140841488386,0.029024700460621052
0.902,0.3194720905597903,0.10751291979009034,0.029210025652070506
0.903,0.32071549125470084,0.10804655504148289,0.02939630523817157
0.904,0.32196250362288514,0.10858232062029026,0.02958354312836833
0.905,0.3232131348257656,0.10912022299147166,0.02977174324433493
0.906,0.32446739351378395,0.10966026863373726,0.02996090952000284
0.907,0.3257252839325883,0.1102024640395642,0.03015104590158791
0.908,0.32698681472155927,0.11074681571521575,0.03034215634761747
0.909,0.32825199307624087,0.11129333018075874,0.030534244828957724
0.91,0.32952082620072554,0.11184201397008302,0.030727315328841088
0.911,0.3307933213076538,0.11239287363091745,0.030921371842893078
0.912,0.33206948561821675,0.11294591572484924,0.031116418379160158
0.913,0.33334932636217035,0.11350114682734196,0.03131245895813683
0.914,0.33463285077783006,0.1140585735277534,0.03150949761279315
0.915,0.3359200661120844,0.1146182024293547,0.03170753838860211
0.916,0.3372109813846783,0.1151800401493463,0.03190658534356702
0.917,0.3385056003597172,0.11574409331887872,0.03210664254824945
0.918,0.3398039320455264,0.1163103685830682,0.03230771408579631
0.919,0.34110598372332085,0.11687887260101713,0.03250980405196776
0.92,0.34241176268291157,0.11744961204583071,0.03271291655516471
0.921,0.34372127622270976,0.1180225936046358,0.03291705571645657
0.922,0.3450345316497314,0.1185978239785988,0.03312222566960896
0.923,0.34635153627960275,0.11917530988294418,0.033328430561111344
0.924,0.34767229743656525,0.11975505804697237,0.033535674550204994
0.925,0.34899682245347974,0.12033707521407828,0.033743961808910795
0.926,0.3503251207245085,0.12092136814176976,0.03395329652205683
0.927,0.35165719552351377,0.12150794360168526,0.03416368288730684
0.928,0.3529930562328755,0.12209680837961223,0.034375125115187505
0.929,0.3543327102199876,0.12268796927550582,0.03458762742911699
0.93,0.3556761648608894,0.12328143310350703,0.034801194065432584
0.931,0.3570234275402707,0.12387720669196055,0.03501582927341899
0.932,0.3583745056514782,0.1244752968834338,0.035231537315336216
0.933,0.3597294065965181,0.12507571053473493,0.03544832246644791
0.934,0.3610881377860636,0.12567845451693052,0.035666189015049324
0.935,0.3624507066394598,0.12628353571536488,0.03588514126249583
0.936,0.3638171229304416,0.1268909610296784,0.036105183523230604
0.937,0.3651873894338405,0.1275007373738252,0.03632632012481356
0.9380000000000001,0.3665615159112453,0.1281128716760919,0.03654855540794934
0.9390000000000001,0.36793950981673645,0.12872737087911615,0.03677189372651543
0.9400000000000001,0.36932137861308834,0.12934424193990463,0.03699633944759108
0.9410000000000001,0.37070712977177855,0.12996349182985256,0.03722189695148563
0.9420000000000001,0.3720967707729923,0.13058512753475973,0.037448570631766334
0.9430000000000001,0.3734903091056237,0.1312091560548521,0.03767655515997614
0.9440000000000001,0.374887752267286,0.13183558440479778,0.03790574062197458
0.9450000000000001,0.37628910776431224,0.13246441961372646,0.03813605721756069
0.9460000000000001,0.3776943857552195,0.13309566872524775,0.03836750940065943
0.9470000000000001,0.37910358850692694,0.13372933879746993,0.0386001016386188
0.9480000000000001,0.38051672616543103,0.1343654369030179,0.03883383841223886
0.9490000000000001,0.3819338062720046,0.13500397012905285,0.03906872421580084
0.9500000000000001,0.3833548363766687,0.13564494557728832,0.039304763557095355
0.9510000000000001,0.3847798240381952,0.13628837036401145,0.03954196095745162
0.9520000000000001,0.3862087768241127,0.13693425162010042,0.03978032095176661
0.9530000000000001,0.3876417023107148,0.13758259649104226,0.04001984808853319
0.9540000000000001,0.38907860808305983,0.13823341213695256,0.04026054692986996
0.9550000000000001,0.3905195017349799,0.13888670573259404,0.04050242205154978
0.9560000000000001,0.3919643938150118,0.139542484467394,0.04074547804302893
0.9570000000000001,0.393413286073206,0.14020075554546352,0.0409897195074763
0.9580000000000001,0.3948661890452055,0.14086152618561654,0.04123515106180245
0.9590000000000001,0.3963231103599857,0.14152480362138783,0.041481777336688695
0.9600000000000001,0.3977840576553175,0.14219059510105195,0.04172960297661642
0.961,0.39924903857777655,0.1428589078876423,0.04197863263989624
0.962,0.40071806078274275,0.14352974925896833,0.0422288709986976
0.963,0.40219113193441525,0.14420312650763503,0.04248032273907772
0.964,0.4036682597058071,0.144879046941063,0.042732992561010756
0.965,0.40514945177875544,0.1455575178815045,0.042986885178418074
0.966,0.4066347190971081,0.1462385466660645,0.043242005319196926
0.967,0.40812406288499137,0.1469221406467174,0.04349835772524995
0.968,0.40961749407298514,0.1476083071903275,0.04375594715251512
0.969,0.4111150203782686,0.14829705367866583,0.04401477837099505
0.97,0.41261664952687327,0.14898838750843152,0.04427485616478657
0.971,0.41412238925368466,0.14968231609126798,0.044536185332110394
0.972,0.41563224730244486,0.1503788468537823,0.04479877068534093
0.973,0.4171462314257616,0.15107798723756544,0.04506261705103547
0.974,0.41866434938511154,0.1517797446992091,0.0453277292699647
0.975,0.42018660895084425,0.15248412671032624,0.04559411219714221
0.976,0.4217130214674494,0.1531911407575677,0.045861770701853696
0.977,0.42324358762399594,0.15390079434264414,0.04613070966768798
0.978,0.4247783187513196,0.15461309498234144,0.04640093399256569
0.979,0.42631722265531924,0.15532805020854135,0.04667244858877033
0.98,0.42786030715079154,0.15604566756824087,0.0469452583829775
0.981,0.42940758006143714,0.15676595462357037,0.04721936831628499
0.982,0.43095904921986805,0.15748891895181147,0.04749478334424349
0.983,0.4325147224676094,0.15821456814541754,0.04777150843688555
0.984,0.4340746076551065,0.1589429098120321,0.04804954857875704
0.985,0.43563871264173043,0.1596739515745073,0.048328908768946036
0.986,0.4372070491779889,0.16040770107092325,0.04860959402111414
0.987,0.4387796174086638,0.16114416595460676,0.048891609363526094
0.988,0.44035642907022415,0.16188335389414935,0.04917495983908016
0.989,0.44193749205779,0.16262527257342949,0.049459650505338466
0.99,0.4435228142754313,0.1633699296916262,0.04974568643455799
0.991,0.44511240363617494,0.16411733296324335,0.050033072713719366
0.992,0.4467062680620042,0.16486749011812588,0.05032181444455935
0.993,0.4483044154838722,0.1656204089014779,0.05061191674360013
0.994,0.4499068538416997,0.1663760970738846,0.050903384742179786
0.995,0.45151359108438316,0.16713456241132907,0.051196223586483215
0.996,0.4531246393738732,0.1678958127052113,0.051490438437573054
0.997,0.4547399983013464,0.16865985576236903,0.051786034471419516
0.998,0.4563596800143205,0.16942669940509408,0.052083016878931604
0.999,0.45798369249764626,0.17019635147115483,0.0523813908659879
1.0,0.4596120437451715,0.17096881981381148,0.05268116165346701

==> wave.tex <==
x,t2,t3,t4
0.001,7.391427292433988e-06,6.838206880698729e-06,6.838206791331375e-06
0.002,8.497504234201663e-06,6.840188416107695e-06,6.840186986222161e-06
0.003,9.600212044081908e-06,6.843494528414559e-06,6.843487283974166e-06
0.004,1.069954953310668e-05,6.84813056436276e-06,6.848107642702591e-06
0.005,1.1795513459173518e-05,6.854104043276299e-06,6.854048005049755e-06
0.006,1.288804302617004e-05,6.8614246128635975e-06,6.8613082965423386e-06
0.007,1.3977230791740826e-05,6.870104135152498e-06,6.8698884261736115e-06
0.008,1.5063022955679204e-05,6.8801565198403856e-06,6.879788286321381e-06
0.009000000000000001,1.6145408066522473e-05,6.891597861711108e-06,6.891007752982483e-06
0.010000000000000002,1.722437261999175e-05,6.90444647004149e-06,6.903546685469724e-06
0.011,1.8299901059125895e-05,6.918723334814569e-06,6.9174049259687795e-06
0.012,1.9371975773410007e-05,6.934450918083052e-06,6.9325823000778865e-06
0.013000000000000001,2.044057709849968e-05,6.951654106311433e-06,6.949078616814329e-06
0.014000000000000002,2.1505683316260998e-05,6.970360398316586e-06,6.966893668080898e-06
0.015,2.256727065421012e-05,6.990598744747139e-06,6.986027228841403e-06
0.016,2.3625146756512573e-05,7.01240028800977e-06,7.006479056851522e-06
0.017,2.467960569277582e-05,7.035798527258928e-06,7.028248893101707e-06
0.018000000000000002,2.5730462101064752e-05,7.060829125546426e-06,7.051336461070955e-06
0.019000000000000003,2.677768398696254e-05,7.087529911062071e-06,7.075741467352995e-06
0.02,2.7821237299871512e-05,7.11594087684315e-06,7.101463600644331e-06
0.021,2.886108593170101e-05,7.146105605613845e-06,7.128502532496398e-06
0.022000000000000002,2.989719171674263e-05,7.17806891134039e-06,7.156857916666725e-06
0.023,3.092951443062398e-05,7.2118761391935795e-06,7.186529389485865e-06
0.024,3.1958011790091914e-05,7.247576033342291e-06,7.21751656927e-06
0.025,3.298263945212439e-05,7.285219510496537e-06,7.249819073926422e-06
0.026000000000000002,3.4003073396569346e-05,7.324859660415482e-06,7.2834364848163104e-06
0.027000000000000003,3.5019809278347425e-05,7.3665517476550405e-06,7.318368531725562e-06
0.028,3.6032530066716814e-05,7.410353211123486e-06,7.354614619142016e-06
0.029,3.7041183172141016e-05,7.456323665771187e-06,7.392174277995536e-06
0.030000000000000002,3.804571394136979e-05,7.504524903431861e-06,7.431047020764554e-06
0.031,3.9046065656413003e-05,7.555020893918457e-06,7.471232341500435e-06
0.032,4.004217953421223e-05,7.607877785408763e-06,7.512729715011937e-06
0.033,4.1033994725067485e-05,7.663163906178187e-06,7.555538597418399e-06
0.034,4.20214483121047e-05,7.72094976513989e-06,7.599658425447452e-06
0.035,4.3004475309673e-05,7.781308053637938e-06,7.6450887277536e-06
0.036000000000000004,4.39826198568105e-05,7.844313645882032e-06,7.691829167141202e-06
0.037000000000000005,4.495657931472083e-05,7.910043600039198e-06,7.739879320932882e-06
0.038,4.5925904804613555e-05,7.97857716040488e-06,7.789238117132406e-06
0.039,4.689052305693262e-05,8.04999575753971e-06,7.83990490342755e-06
0.04,4.7850358727959654e-05,8.124400345498598e-06,7.891879007749434e-06
0.041,4.880533439928929e-05,8.201864992996856e-06,7.945159737365853e-06
0.042,4.975537057533365e-05,8.282474875899445e-06,7.999746379961528e-06
0.043000000000000003,5.070038568374141e-05,8.366320346331146e-06,8.055638379915363e-06
0.044000000000000004,5.164029607281014e-05,8.453493954242133e-06,8.112835052111407e-06
0.045,5.257501601058924e-05,8.544090448408977e-06,8.171335724613598e-06
0.046,5.350395754778507e-05,8.638206777568175e-06,8.231139431626462e-06
0.047,5.4428019917517635e-05,8.735942092792609e-06,8.292245274696766e-06
0.048,5.5346622143071756e-05,8.837397748413462e-06,8.354652419087528e-06
0.049,5.625967015805562e-05,8.942677303041846e-06,8.418360258095902e-06
0.05,5.716706780761415e-05,9.05188652302e-06,8.483368065506665e-06
0.051000000000000004,5.8068716848959235e-05,9.165133381819061e-06,8.54967561622346e-06
0.052000000000000005,5.896451694800545e-05,9.282528063749122e-06,8.617281196609287e-06
0.053000000000000005,5.9854365679227445e-05,9.404182964033603e-06,8.686183761330428e-06
0.054,6.0738158522691285e-05,9.530212692050065e-06,8.756382350973049e-06
0.055,6.161578886372853e-05,9.660734071702845e-06,8.82787749918696e-06
0.056,6.248653634390562e-05,9.795866144317003e-06,8.900666852309708e-06
0.057,6.335150228265789e-05,9.935730169951763e-06,8.974750832223465e-06
0.058,6.420997328232017e-05,1.0080449629733934e-05,9.050129000498958e-06
0.059000000000000004,6.506183432929018e-05,1.023015022713837e-05,9.126798730658565e-06
0.060000000000000005,6.590696830552168e-05,1.0384959890639746e-05,9.204758733422843e-06
0.061,6.674525598697105e-05,1.0545008775374607e-05,9.284007965690668e-06
0.062,6.757657604170497e-05,1.0710429265174927e-05,9.364545444648988e-06
0.063,6.840080502775615e-05,1.0881355974898797e-05,9.446369816170484e-06
0.064,6.921781739154687e-05,1.1057925752101977e-05,9.529479895423833e-06
0.065,7.002748546550381e-05,1.1240277679644363e-05,9.613874471731697e-06
0.066,7.082895608974434e-05,1.1428553077304874e-05,9.699553299430181e-06
0.067,7.162353292988699e-05,1.1622895504637942e-05,9.786514590756028e-06
0.068,7.241036977158867e-05,1.1823450763280872e-05,9.87475669832047e-06
0.069,7.318933047191706e-05,1.203036689804221e-05,9.964281388742642e-06
0.07,7.396027676278236e-05,1.2243794201004388e-05,1.0055088441603665e-05
0.07100000000000001,7.472306825027823e-05,1.246388521225185e-05,1.0147173626730948e-05
0.07200000000000001,7.547756241140397e-05,1.2690794723415294e-05,1.0240535261239942e-05
0.07300000000000001,7.622361459216887e-05,1.2924679779657205e-05,1.0335172321682125e-05
0.074,7.696107800567996e-05,1.316569968179305e-05,1.0431082933964664e-05
0.075,7.76898037289885e-05,1.341401598961572e-05,1.0528265359281831e-05
0.076,7.840880533401374e-05,1.3669792523756301e-05,1.0626718108295041e-05
0.077,7.911958913981245e-05,1.393319536823058e-05,1.0726439661458035e-05
0.078,7.982354146316617e-05,1.4204392874035221e-05,1.0827428469563747e-05
0.079,8.05187971905309e-05,1.4483555660279216e-05,1.0929683897944211e-05
0.08,8.120462574038894e-05,1.4770856617985139e-05,1.103320442004374e-05
0.081,8.188086588684704e-05,1.506647091260155e-05,1.1137987489196359e-05
0.082,8.254735425893699e-05,1.5370575986267034e-05,1.1244031434079628e-05
0.083,8.320392533715207e-05,1.568335156154012e-05,1.1351341517556231e-05
0.084,8.385041145192183e-05,1.600497964299715e-05,1.1459916600110818e-05
0.085,8.448664277973554e-05,1.6335644521460496e-05,1.1569748541877442e-05
0.08600000000000001,8.511150197314767e-05,1.667553277547033e-05,1.168083528388283e-05
0.08700000000000001,8.5726694411293e-05,1.7024833275530884e-05,1.1793175151893659e-05
0.08800000000000001,8.633110964281655e-05,1.738373718613565e-05,1.190676642216536e-05
0.089,8.692456920376256e-05,1.775243796951866e-05,1.2021606999679511e-05
0.09,8.75068924631719e-05,1.8131131388195215e-05,1.2137695257641194e-05
0.091,8.807789662025602e-05,1.852001550798592e-05,1.2255028999914163e-05
0.092,8.863739670109463e-05,1.891929070159765e-05,1.2373606223922563e-05
0.093,8.918520555593314e-05,1.9329159651499497e-05,1.2493425096521483e-05
0.094,8.972186409550744e-05,1.974982735322338e-05,1.2614494828581374e-05
0.095,9.024669964301297e-05,2.0181501118407724e-05,1.2736802517067622e-05
0.096,9.075817796651555e-05,2.062439057827738e-05,1.2860346048537787e-05
0.097,9.125821159796266e-05,2.1078707686903477e-05,1.2985123271357435e-05
0.098,9.174555313978578e-05,2.1544666724455412e-05,1.3111131995085022e-05
0.099,9.222000181411328e-05,2.2022484300865758e-05,1.3238369990203542e-05
0.1,9.268135464033702e-05,2.2512379358759847e-05,1.3366834987162987e-05
0.101,9.312940643127759e-05,2.3014573177547566e-05,1.3496524727131303e-05
0.10200000000000001,9.356394979064445e-05,2.35292893761372e-05,1.3627436962582649e-05
0.10300000000000001,9.39847751088711e-05,2.4056753917463325e-05,1.3759569161933724e-05
0.10400000000000001,9.439167056057961e-05,2.459719511112071e-05,1.3892918891823615e-05
0.10500000000000001,9.478442210059011e-05,2.5150843617667586e-05,1.4027483827514444e-05
0.106,9.516164037095133e-05,2.5717932451580082e-05,1.4163261515386914e-05
0.107,9.552544173561214e-05,2.6298696985947626e-05,1.4300249201905126e-05
0.108,9.587444369791718e-05,2.689337495504258e-05,1.4438444281425051e-05
0.109,9.62084233002399e-05,2.7502206458843543e-05,1.4577844103836314e-05
0.11,9.652715534764914e-05,2.8125433967048873e-05,1.471844597409999e-05
0.111,9.683041240541337e-05,2.8763302321737572e-05,1.4860247150597727e-05
0.112,9.71179647938745e-05,2.9416058742848772e-05,1.5003244846013917e-05
0.113,9.738958058598868e-05,3.008395283080693e-05,1.514743622554554e-05
0.114,9.764502560314724e-05,3.0767236571032836e-05,1.5292818406769995e-05
0.115,9.788469646947377e-05,3.146616433799181e-05,1.5439388459127304e-05
0.116,9.810942055930918e-05,3.2180992899045e-05,1.558714340308676e-05
0.117,9.83186161967763e-05,3.2911981418917946e-05,1.5736080209901776e-05
0.11800000000000001,9.851076896380981e-05,3.365939146285275e-05,1.5886195800093116e-05
0.11900000000000001,9.868563421098533e-05,3.442348700190524e-05,1.6037487043861295e-05
0.12000000000000001,9.884296502210425e-05,3.520453441676717e-05,1.618995076009486e-05
0.121,9.898251221057994e-05,3.600280250162596e-05,1.6343583715361863e-05
0.122,9.910402431524844e-05,3.681856246868782e-05,1.6498386175880343e-05
0.123,9.920724759621331e-05,3.7652087952599025e-05,1.66543541315487e-05
0.124,9.929192603081333e-05,3.8503655014789804e-05,1.681148175807119e-05
0.125,9.935780130972889e-05,3.937354214767564e-05,1.696976546850514e-05
0.126,9.940321586505742e-05,4.026203027961e-05,1.7129201767624497e-05
0.127,9.94306893491784e-05,4.116940277815157e-05,1.7289787103477112e-05
0.128,9.943857098171757e-05,4.2095945456418494e-05,1.74515178684203e-05
0.129,9.942659326454606e-05,4.3041946575883116e-05,1.761439039680887e-05
0.13,9.939448639151097e-05,4.400769685190824e-05,1.7778400965128214e-05
0.131,9.93419782441318e-05,4.4993489458378864e-05,1.7943545791278814e-05
0.132,9.92687943876393e-05,4.599962003191565e-05,1.810982103346589e-05
0.133,9.91746580659615e-05,4.702638667729321e-05,1.827722371137008e-05
0.134,9.905929019795585e-05,4.8074089971438456e-05,1.8445749287867853e-05
0.135,9.892240937260489e-05,4.9143032968620754e-05,1.8615393458250722e-05
0.136,9.876222077077131e-05,5.02335212055532e-05,1.8786152138102842e-05
0.137,9.858144901527796e-05,5.134586270549325e-05,1.8958021179478134e-05
0.138,9.837830603901576e-05,5.248036798416159e-05,1.913099637101064e-05
0.139,9.815250106580562e-05,5.363735005407478e-05,1.9305073436620353e-05
0.14,9.790374096694304e-05,5.481712442933354e-05,1.9480248034517634e-05
0.14100000000000001,9.763173025563205e-05,5.602000913165391e-05,1.9656515757322534e-05
0.14200000000000002,9.733617108311163e-05,5.72463246944882e-05,1.983387213038551e-05
0.14300000000000002,9.70167632334849e-05,5.849639416855603e-05,2.0012312611385984e-05
0.14400000000000002,9.667507031350904e-05,5.977054312710209e-05,2.0191832589566237e-05
0.14500000000000002,9.631142547563643e-05,6.106909967094005e-05,2.0372427384800314e-05
0.146,9.592241109888736e-05,6.239239443363508e-05,2.0554092246710528e-05
0.147,9.551386205411148e-05,6.374076058726168e-05,2.0736822354228617e-05
0.148,9.50801580342796e-05,6.51145338474236e-05,2.0920612814518985e-05
0.149,9.462098695796677e-05,6.651405247851031e-05,2.1105460664280768e-05
0.15,9.41377772887101e-05,6.793965729934972e-05,2.12913895770755e-05
0.151,9.363133952483546e-05,6.939169168869722e-05,2.1478380932825428e-05
0.152,9.309858455133656e-05,7.087050159092101e-05,2.1666414242673027e-05
0.153,9.253919178897404e-05,7.237643552081276e-05,2.185548428370447e-05
0.154,9.195283826234196e-05,7.39098445703174e-05,2.2045585757313188e-05
0.155,9.133919859533777e-05,7.547108241342188e-05,2.2236713287645357e-05
0.156,9.069621993680247e-05,7.706050531178484e-05,2.2428861420658698e-05
0.157,9.002701077894449e-05,7.867847212096236e-05,2.262202462370231e-05
0.158,8.933490304307937e-05,8.032534429630005e-05,2.281619728469015e-05
0.159,8.861552979180509e-05,8.20014858977614e-05,2.3011373710355807e-05
0.16,8.787459347364133e-05,8.370726359689791e-05,2.3207595715416517e-05
0.161,8.710822976237825e-05,8.54430466823468e-05,2.3404823057804337e-05
0.162,8.631651441369131e-05,8.72092070656724e-05,2.3603038655742186e-05
0.163,8.550049298786824e-05,8.900611928761296e-05,2.3802236522992015e-05
0.164,8.465825983500081e-05,9.083416052401116e-05,2.400241282973641e-05
0.165,8.378599492330445e-05,9.269371059184817e-05,2.4203560587780953e-05
0.166,8.288154170113974e-05,9.458515195555043e-05,2.4405698663665165e-05
0.167,8.195199289804541e-05,9.650886973296751e-05,2.460883838928614e-05
0.168,8.09915609112115e-05,9.84652517020245e-05,2.481293161347841e-05
0.169,7.999977807407365e-05,0.00010045468830658767,2.5017971871730064e-05
0.17,7.898000429245496e-05,0.00010247757266284156,2.5223952609594443e-05
0.171,7.793524605366799e-05,0.00010453430056566364,2.5430932694423643e-05
0.17200000000000001,7.685829085659177e-05,0.00010662527049568044,2.563890158681729e-05
0.17300000000000001,7.574877906821713e-05,0.00010875088362443338,2.5847807173669712e-05
0.17400000000000002,7.460777102311029e-05,0.00011091154382216144,2.6057630600846648e-05
0.17500000000000002,7.343908124201234e-05,0.00011310765766387974,2.6268364926728375e-05
0.17600000000000002,7.223498780602186e-05,0.00011533963443572618,2.6480003114541452e-05
0.177,7.100961341253105e-05,0.00011760788614190214,2.669253803152702e-05
0.178,6.97591995742415e-05,0.00011991282751135101,2.690596244793424e-05
0.179,6.848985744043705e-05,0.00012225487600474368,2.712026903622917e-05
0.18,6.720810941866912e-05,0.00012463445182050949,2.7335450369326856e-05
0.181,6.592244196732592e-05,0.00012705197790268509,2.755149892050356e-05
0.182,6.46124528522166e-05,0.00012950787994706742,2.776840706164965e-05
0.183,6.328747005565832e-05,0.00013200258640856509,2.798616706261288e-05
0.184,6.194614722371039e-05,0.000134536528507763,2.8204771089725304e-05
0.185,6.058096485523523e-05,0.00013711014023851394,2.842421218829356e-05
0.186,5.919637866340668e-05,0.000139723858374676,2.8644488080866856e-05
0.187,5.779956701167465e-05,0.00014237812247725967,2.8865584195816724e-05
0.188,5.6384810772612636e-05,0.00014507337490162554,2.9087492284254595e-05
0.189,5.497774428760535e-05,0.0001478100608051242,2.9310203989085252e-05
0.19,5.358591578531225e-05,0.00015058862815344267,2.9533710843046233e-05
0.191,5.2230291629848206e-05,0.00015340952772920815,2.975800426874268e-05
0.192,5.0900370290452445e-05,0.00015627321313796047,2.9983081785641286e-05
0.193,4.9600413776941095e-05,0.00015918014081704165,3.020893138585719e-05
0.194,4.8330150891067314e-05,0.000162130770041875,3.043564669961036e-05
0.195,4.708617267083666e-05,0.00016512556293400436,3.066315727602376e-05
0.196,4.593993025091056e-05,0.000168164984469112,3.089141435582145e-05
0.197,4.492023686360167e-05,0.00017124950248354105,3.112040874401627e-05
0.198,4.3973716100964334e-05,0.00017437958768319798,3.1350131128059226e-05
0.199,4.3110673282269386e-05,0.00017755571365062831,3.158059635874548e-05
0.2,4.234368114311226e-05,0.00018077835685263504,3.1811879184573245e-05
0.201,4.17115403571917e-05,0.00018404799664861868,3.2043940809071766e-05
0.202,4.120097850297784e-05,0.00018736511529843895,3.227674832719455e-05
0.203,4.083632352504656e-05,0.00019073019796995557,3.251024284433714e-05
0.20400000000000001,4.062057409440453e-05,0.00019414373274718379,3.27444337464678e-05
0.20500000000000002,4.055853190902361e-05,0.00019760621063870558,3.297931387571447e-05
0.20600000000000002,4.062485952442296e-05,0.000201118125585355,3.321485198172439e-05
0.20700000000000002,4.085024660559851e-05,0.00020467997446831706,3.345110246719065e-05
0.20800000000000002,4.123065972983961e-05,0.00020829225711780874,3.368799841968916e-05
0.20900000000000002,4.1748491468609395e-05,0.00021195547632089535,3.3925523120707916e-05
0.21,4.242711725037542e-05,0.0002156701378301758,3.416366591951759e-05
0.211,4.330357804900103e-05,0.00021943675037175664,3.440241782702429e-05
0.212,4.431332394434189e-05,0.00022325582565384033,3.464187411989352e-05
0.213,4.543868467376684e-05,0.00022712787837541855,3.4882087123366304e-05
0.214,4.6729772678716724e-05,0.0002310534262345926,3.512311308212435e-05
0.215,4.817709348976249e-05,0.00023503298993694146,3.536492386879822e-05
0.216,4.9805433927740306e-05,0.0002390670932047585,3.560730745098205e-05
0.217,5.1652052169614e-05,0.00024315626278530801,3.585036666626311e-05
0.218,5.367983218532671e-05,0.0002473010284594087,3.6094005129103004e-05
0.219,5.5901258637805216e-05,0.0002515019230510112,3.633818432005837e-05
0.22,5.8304654192900185e-05,0.00025575948243502903,3.6583059557272334e-05
0.221,6.0873546349793e-05,0.0002600742455471269,3.682845891163027e-05
0.222,6.355858721394142e-05,0.00026444675439225856,3.707436932882383e-05
0.223,6.637217633925485e-05,0.00026887755405385314,3.732078946767934e-05
0.224,6.932186818547147e-05,0.00027336719270277106,3.7567695744236625e-05
0.225,7.240141517515719e-05,0.00027791622160665524,3.7815075858716454e-05
0.226,7.561101588377276e-05,0.000282525195138791,3.8062981805500156e-05
0.227,7.896239571871736e-05,0.00028719467078790694,3.8311660345660124e-05
0.228,8.241727311202934e-05,0.0002919252091668321,3.856097330897005e-05
0.229,8.597635515399308e-05,0.00029671737402255295,3.8810757819760154e-05
0.23,8.967077608915769e-05,0.0003015717322449222,3.906096795503468e-05
0.231,9.346531821967723e-05,0.00030648885387690847,3.9311837733134764e-05
0.232,9.73543477006721e-05,0.0003114693121236819,3.956333468156425e-05
0.233,0.0001013506929875425,0.0003165136833621607,3.9815229638697697e-05
0.234,0.00010546327703885695,0.0003216225471510056,4.006750932001973e-05
0.23500000000000001,0.00010967991684796816,0.0003267964862400389,4.0320163911742246e-05
0.23600000000000002,0.00011401052981019135,0.00033203608658044254,4.057317976914171e-05
0.23700000000000002,0.00011843210743252844,0.0003373419373341311,4.082653980659222e-05
0.23800000000000002,0.0001229426874685755,0.00034271463088397385,4.108023011259398e-05
0.23900000000000002,0.00012753552426877248,0.0003481547628434584,4.13342366138715e-05
0.24000000000000002,0.00013220618515027126,0.00035366293206730775,4.158854507446443e-05
0.241,0.00013696314262187263,0.0003592397406608719,4.1843141093601035e-05
0.242,0.00014180322726346144,0.0003648857939907239,4.209811435763831e-05
0.243,0.0001467208346951838,0.00037060170069468296,4.235350900376635e-05
0.244,0.00015173020572757605,0.00037638807269239346,4.260920345085093e-05
0.245,0.0001568269761032329,0.00038224552519511133,4.2865510357683656e-05
0.246,0.00016200652868140407,0.00038817467671664927,4.312204717122933e-05
0.247,0.00016726489213043987,0.0003941761490835637,4.3379277790388246e-05
0.248,0.00017260319836208906,0.0004002505674455396,4.3637064813582726e-05
0.249,0.00017802784857898758,0.0004063985602865188,4.389543831035721e-05
0.25,0.0001835359033683829,0.000412620759434726,4.415408934544897e-05
0.251,0.0001891247059260966,0.0004189178000738371,4.441363562379103e-05
0.252,0.00019479968960884128,0.0004252903207533939,4.467342900799135e-05
0.253,0.00020056485839243423,0.0004317389634000321,4.493341066554061e-05
0.254,0.00020641218359140358,0.00043826437332815464,4.519361377406917e-05
0.255,0.00021234078129154696,0.0004448671992509387,4.545395746985177e-05
0.256,0.00021835234087439812,0.0004515480932913077,4.571442567310787e-05
0.257,0.00022444127719251886,0.00045830771099323757,4.5975581250728585e-05
0.258,0.00023061136211821893,0.00046514671133277534,4.623712370477741e-05
0.259,0.0002368632575257957,0.0004720657567293456,4.649879208582505e-05
0.26,0.00024319762875753555,0.00047906551305686894,4.6760667900618444e-05
0.261,0.00024961514463559025,0.0004861466496554628,4.702275901068631e-05
0.262,0.00025611647747313316,0.0004933098393427167,4.728504805516443e-05
0.263,0.00026270230308578186,0.0005005557584249827,4.7547375758195715e-05
0.264,0.00026937330080340833,0.0005078850867093085,4.78098288574126e-05
0.265,0.0002761301534816798,0.0005152985075148208,4.807243430062818e-05
0.266,0.0002829768070546163,0.000522796707684723,4.83350321208616e-05
0.267,0.0002899074457368352,0.0005303803775976566,4.859760468603883e-05
0.268,0.000296926009231725,0.0005380502111798901,4.886013417155119e-05
0.269,0.0003040331946161968,0.0005458069059170405,4.912260255849905e-05
0.27,0.00031122970255241495,0.000553651162866261,4.938499163219792e-05
0.271,0.0003185162372996055,0.0005615836866681036,4.964728298036918e-05
0.272,0.0003258935067264192,0.000569605185558712,4.9909952423436985e-05
0.273,0.000333362222322977,0.0005777163713820493,5.017256625160398e-05
0.274,0.0003409230992131958,0.0005859179596020087,5.043503818333936e-05
0.275,0.0003485768561674005,0.0005942106693152058,5.069736415220624e-05
0.276,0.00035632760925400107,0.0006025952232626913,5.096050661838681e-05
0.277,0.0003641693107733118,0.000611072347842993,5.122369947599146e-05
0.278,0.0003721060706818072,0.0006196427731245938,5.148681584698379e-05
0.279,0.00038013862245926694,0.0006283072328582082,5.174972309416006e-05
0.28,0.000388267703294811,0.0006370664644899692,5.201240149591301e-05
0.281,0.00039649405409919024,0.0006459212091738355,5.2274831120917756e-05
0.28200000000000003,0.0004048184195178676,0.000654872211784486,5.2536991826438165e-05
0.28300000000000003,0.00041324154794405857,0.000663920220930579,5.2799170902412475e-05
0.28400000000000003,0.0004217641915315059,0.000673065988967255,5.306119441790693e-05
0.28500000000000003,0.0004303871062076649,0.0006823102720095206,5.332318231883511e-05
0.28600000000000003,0.0004391145807171177,0.0006916538299454412,5.358501697481994e-05
0.28700000000000003,0.0004479403341265537,0.0007010974264491,5.3846894393318764e-05
0.28800000000000003,0.00045686864919531397,0.0007106418289940919,5.41087257907427e-05
0.28900000000000003,0.00046590029707832374,0.0007202878088668353,5.437051025133163e-05
0.29,0.00047503605277084035,0.0007300361411801074,5.4632309147727527e-05
0.291,0.00048427669512194824,0.0007398876048864024,5.489388042812115e-05
0.292,0.0004936230068482305,0.0007498429827917142,5.515517451104272e-05
0.293,0.0005030757745475058,0.0007599030615691191,5.5416280076705507e-05
0.294,0.0005126357887124168,0.0007700686317724964,5.567749589779267e-05
0.295,0.000522303843744693,0.0007803404878505972,5.593849453901806e-05
0.296,0.0005320844037382405,0.0007907194281607492,5.619924015408295e-05
0.297,0.000541970953165413,0.0008012062549827334,5.6459759671725695e-05
0.298,0.0005519679502716532,0.0008118017745333487,5.6719767925708676e-05
0.299,0.0005620762052340461,0.0008225067969799723,5.697923062868022e-05
0.3,0.0005722965322091288,0.0008333221364553147,5.723821930693233e-05
0.301,0.0005826297493470167,0.0008442486110713224,5.749786737348887e-05
0.302,0.0005930766788060796,0.0008552870429340291,5.775750462320637e-05
0.303,0.0006036381467671514,0.0008664382581575737,5.80165414776852e-05
0.304,0.0006143149834482186,0.000877703086879015,5.827553776410024e-05
0.305,0.0006251080231192002,0.0008890823632729478,5.8534260322790484e-05
0.306,0.0006360219080345628,0.0009005769255663833,5.8793209131776205e-05
0.307,0.0006470498866711642,0.0009121876160532737,5.905204530772751e-05
0.308,0.0006581965955811858,0.000923915281109451,5.93102123634764e-05
0.309,0.0006694628853906077,0.0009357607712080273,5.956800518316667e-05
0.31,0.0006808496108515335,0.0009477249409338052,5.9825357132486335e-05
0.311,0.0006923576308579445,0.0009598086489990725,6.008203587334172e-05
0.312,0.0007039878084606249,0.0009720127582583483,6.03382219653524e-05
0.313,0.0007157410108825361,0.0009843381357239258,6.059421839016376e-05
0.314,0.000727618109534558,0.0009967856525814032,6.085118956001898e-05
0.315,0.0007396199800306224,0.0010093561842049634,6.110829288682959e-05
0.316,0.0007517514457394217,0.0010220506101730478,6.13654079642636e-05
0.317,0.0007640055177014543,0.0010348698142839492,6.162186021179855e-05
0.318,0.0007763870137406831,0.0010478146845717756,6.187751775584478e-05
0.319,0.0007888968264409739,0.001060886113322154,6.213298495903081e-05
0.32,0.0008015358526684773,0.0010740849970882285,6.238774890479508e-05
0.321,0.0008143049935872396,0.0010874122367064633,6.264185876325967e-05
0.322,0.0008272051546761074,0.0011008687373132836,6.289655863055797e-05
0.323,0.0008402372457442136,0.0011144554083607516,6.31527031154341e-05
0.324,0.0008534021809477095,0.0011281731636330985,6.340865899064423e-05
0.325,0.000866700878806102,0.0011420229212631872,6.36637260944072e-05
0.326,0.0008801383469045778,0.001156005603748842,6.391902052789852e-05
0.327,0.00089370735736902,0.0011701221379695828,6.41746477891305e-05
0.328,0.0009074129124085212,0.0011843734552030758,6.443082789948004e-05
0.329,0.0009212559481621923,0.0011987604911422726,6.468725715161673e-05
0.33,0.0009352374052157895,0.0012132841859117882,6.494361536766789e-05
0.331,0.0009493582286192003,0.0012279454840853844,6.520052319229117e-05
0.332,0.0009636193679028349,0.0012427453347024428,6.545813996706154e-05
0.333,0.000978021777095493,0.0012576846912856303,6.571609634121848e-05
0.334,0.00099256641474115,0.0012727645118578313,6.597315514236755e-05
0.335,0.0010072542439165742,0.0012879857589595542,6.622984790037752e-05
0.336,0.0010220904596804385,0.0013033493996665617,6.64861722965125e-05
0.337,0.0010370675937289063,0.0013188564056070004,6.674178210280348e-05
0.338,0.0010521908359255687,0.0013345077529794186,6.699758423755342e-05
0.339,0.001067461167653768,0.0013503044225702697,6.72526989678516e-05
0.34,0.0010828795749177485,0.0013662473997717716,6.75072544021637e-05
0.341,0.001098447048360995,0.0013823376746000425,6.776116868762522e-05
0.342,0.0011141645832837403,0.0013985762417127665,6.80150782270379e-05
0.343,0.0011300331796616186,0.0014149641004276214,6.826876330029164e-05
0.34400000000000003,0.0011460538421635906,0.0014315022547403404,6.852169047936368e-05
0.34500000000000003,0.0011622275801706763,0.0014481917133433227,6.877365678265509e-05
0.34600000000000003,0.0011785597796328325,0.0014650334896435743,6.902472796713293e-05
0.34700000000000003,0.0011950427302669284,0.001482028601781695,6.927465121998541e-05
0.34800000000000003,0.0012116818130221358,0.0014991780726503361,6.952348690346716e-05
0.34900000000000003,0.0012284780563123565,0.001516482929912888,6.977202612368528e-05
0.35000000000000003,0.0012454324933568277,0.0015339442060225187,7.002129366443253e-05
0.35100000000000003,0.001262546162198817,0.0015515629382409607,7.027131287896317e-05
0.35200000000000004,0.001279820105725036,0.0015693401686576818,7.052033042645223e-05
0.353,0.0012972553716845288,0.0015872769442089542,7.076857668970327e-05
0.354,0.0013148530127082027,0.0016053743166971443,7.101710144517867e-05
0.355,0.0013326140863282245,0.0016236333428102745,7.126554279704988e-05
0.356,0.0013505441729723447,0.0016420550841411926,7.151449773906578e-05
0.357,0.001368635318795297,0.0016606406072075402,7.176319915255779e-05
0.358,0.0013868930994320157,0.00167939098347105,7.201145748356694e-05
0.359,0.0014053185922159412,0.0016983072893577934,7.226143334915397e-05
0.36,0.0014239128794804655,0.0017173906062778294,7.251194815103513e-05
0.361,0.0014426770485788754,0.0017366420206453204,7.276180728222873e-05
0.362,0.0014616121919047201,0.00175606262389861,7.301137137991153e-05
0.363,0.0014807194069120578,0.001775653512520711,7.325996470652868e-05
0.364,0.001499999796135859,0.0017954157880593913,7.350811310573802e-05
0.365,0.0015194544672125845,0.0018153505571479817,7.375841489287316e-05
0.366,0.00153908919880933,0.0018354589315256159,7.401006872741515e-05
0.367,0.0015588957919051203,0.0018557420280582537,7.426188517708097e-05
0.368,0.0015788800205975902,0.0018762009687594632,7.45145099643943e-05
0.369,0.0015990430131364813,0.001896836880811176,7.476774786005379e-05
0.37,0.0016193859029776077,0.0019176508965850752,7.502262318304762e-05
0.371,0.001639909828803677,0.0019386441536634437,7.527704833961419e-05
0.372,0.0016606159345457997,0.0019598177948607497,7.553133974367027e-05
0.373,0.0016815053694050769,0.001981172968244963,7.578438799547842e-05
0.374,0.00170257928787391,0.0020027108271590552,7.603696718667405e-05
0.375,0.001723838849757824,0.002024432530242599,7.628895837893674e-05
0.376,0.0017452900359084763,0.002046339241453928,7.654106836258947e-05
0.377,0.0017669244004871391,0.0020684321300914995,7.679321740035582e-05
0.378,0.0017887479200149176,0.0020907123708163145,7.704634480402475e-05
0.379,0.001810761775769695,0.0021131811436740553,7.730086009225985e-05
0.38,0.0018329671544525152,0.002135839634117005,7.755741088757379e-05
0.381,0.0018553652482107463,0.002158689033026998,7.78165766782527e-05
0.382,0.001877957254659917,0.0021817305367373835,7.807724205149773e-05
0.383,0.0019007443769069692,0.0022049653470560824,7.834349968256517e-05
0.384,0.0019237278235728476,0.0022283946712882588,7.861096751235073e-05
0.385,0.0019469088088153626,0.002252019722259021,7.887941106529162e-05
0.386,0.0019702935198074104,0.002275841718336862,7.914929911649212e-05
0.387,0.001993873262224361,0.002299861883456335,7.942414807066336e-05
0.388,0.0020176542191650097,0.002324081447141692,7.970246582188079e-05
0.389,0.0020416376271673036,0.0023485016445302636,7.998348022863275e-05
0.39,0.0020658247284228324,0.0023731237163959213,8.026704263176294e-05
0.391,0.002090216770800354,0.002397948909172668,8.055401618028667e-05
0.392,0.002114815007870041,0.0024229784749786503,8.084178462411063e-05
0.393,0.0021396206989273032,0.0024482136716401305,8.113262204837481e-05
0.394,0.0021646351090167924,0.0024736557627152715,8.142594863107562e-05
0.395,0.002189859508956894,0.0024993060175187757,8.171944045805602e-05
0.396,0.0022153002965793235,0.002525165711145752,8.2013254311253e-05
0.397,0.002240948527382066,0.002551236124496678,8.231029857853339e-05
0.398,0.0022668105953978133,0.0025775185443017005,8.260743137319173e-05
0.399,0.002292887794784737,0.002604014263145529,8.290614627203036e-05
0.4,0.002319181425598209,0.0026307245794924034,8.320596194760489e-05
0.401,0.0023456927938153974,0.0026576507977108805,8.350672134298514e-05
0.402,0.0023724232113610725,0.0026847942280993817,8.3810441674043e-05
0.403,0.0023993739961324363,0.0027121561869111782,8.411587800154217e-05
0.404,0.0024265464720250917,0.002739737996380067,8.442203642965881e-05
0.405,0.0024539419689582937,0.0027675409847458454,8.473224783660196e-05
0.406,0.002481567099970906,0.0027955664862802853,8.504836285266618e-05
0.40700000000000003,0.0025094126686716176,0.0028238158413125955,8.53671832497849e-05
0.40800000000000003,0.002537485284594795,0.002852290396256075,8.569480801638873e-05
0.40900000000000003,0.002565786302014646,0.0028809915036337084,8.60271443746389e-05
0.41000000000000003,0.0025943170813598933,0.0029099205221048813,8.636164353956893e-05
0.41100000000000003,0.0026230789892400922,0.002939078816491701,8.669802479935662e-05
0.41200000000000003,0.0026520733984721425,0.0029684677578055976,8.703691239875269e-05
0.41300000000000003,0.00268130168810766,0.0029980887232743513,8.737970505452868e-05
0.41400000000000003,0.0027107652434591885,0.003027943096368588,8.77246845264146e-05
0.41500000000000004,0.0027404654561281614,0.0030580322668293477,8.807112708519749e-05
0.41600000000000004,0.002770409159128752,0.0030883576306949584,8.842296914573533e-05
0.41700000000000004,0.0028005869024521728,0.0031189205903285606,8.87853702619992e-05
0.418,0.002831005515923961,0.0031497225544457057,8.915246575398489e-05
0.419,0.0028616664165737986,0.0031807649381418632,8.952782752448006e-05
0.42,0.0028925710278578706,0.0032120491629205206,8.990828785632715e-05
0.421,0.002923720779686971,0.0032435766567210193,9.029582849747696e-05
0.422,0.002955117108454479,0.0032753488539467406,9.06865367240051e-05
0.423,0.0029867614570651207,0.0033073671954934897,9.108329637105371e-05
0.424,0.0030186552749631563,0.0033396331287779773,9.148779354701594e-05
0.425,0.003050800018161309,0.003372148107766348,9.190049249956855e-05
0.426,0.003083202744649431,0.0034049135930032046,9.231597850266053e-05
0.427,0.003115853749059528,0.0034379310516403716,9.27355843597877e-05
0.428,0.0031487600865310887,0.0034712019574660914,9.315896006115509e-05
0.429,0.003181923239640851,0.0035047277909344165,9.358470904580513e-05
0.43,0.003215344697679711,0.0035385100391945434,9.401247172563713e-05
0.431,0.003249025956682744,0.0035725501961204995,9.444526765428835e-05
0.432,0.003282968519458943,0.0036068497623409786,9.488791892156368e-05
0.433,0.0033171738956210804,0.003641410245269217,9.533801730512045e-05
0.434,0.0033516436016162152,0.0036762331591331686,9.57921123446097e-05
0.435,0.003386379160755758,0.003711320025005869,9.625064011050053e-05
0.436,0.003421387861248439,0.003746672370835832,9.671445703547054e-05
0.437,0.0034566597406163967,0.00378229173147778,9.7183318212032e-05
0.438,0.003492202084580873,0.003818179648723379,9.766093124261051e-05
0.439,0.0035280164442184235,0.0038543376713322058,9.814575732336326e-05
0.44,0.0035641043776247702,0.003890767355063154,9.86330467161082e-05
0.441,0.0036004674499457807,0.003927470262705518,9.91224536869359e-05
0.442,0.003637107233409405,0.003964447964110638,9.961654630798686e-05
0.443,0.0036740253073571784,0.004001702036223626,0.00010012021377003219
0.444,0.003711223258276444,0.004039234063115211,0.00010063392272965467
0.445,0.003748702679832187,0.004077045636013823,0.00010115507649899201
0.446,0.0037864710959507573,0.004115138353337917,0.00010168483718045668
0.447,0.0038245182852895457,0.004153513820728224,0.0001022200901158331
0.448,0.0038628517696762538,0.0041921736510805545,0.00010276525411242524
0.449,0.0039014731718122345,0.004231119464578533,0.00010331334625406476
0.45,0.003940384121740166,0.004270352888726596,0.00010386811490056808
0.451,0.0039795862568771986,0.004309875558383142,0.0001044294260222243
0.452,0.004019081222048334,0.0043496891157939616,0.00010499872561591741
0.453,0.004058870669520243,0.004389795210625721,0.00010557902030897412
0.454,0.004098956259034893,0.004430195499999836,0.0001061734558916434
0.455,0.004139339657843705,0.004470891648526245,0.00010678263466127471
0.456,0.004180028631358087,0.004511885328337678,0.00010739938967265156
0.457,0.004221012697616702,0.004553178219124005,0.00010802013934218444
0.458,0.0042622996203492405,0.004594772008166628,0.00010864554806520664
0.459,0.004303891097188869,0.0046366683903733075,0.0001092805346100904
0.46,0.004345788833451122,0.004678869068313166,0.0001099306283407163
0.461,0.004387994542169129,0.004721375752251568,0.00011058915843012616
0.462,0.004430509944128976,0.004764190160185712,0.00011125671287586119
0.463,0.004473336767905513,0.0048073140178800135,0.00011194074881165503
0.464,0.004516476749897862,0.0048507490589018935,0.00011263885712533814
0.465,0.004559931634365636,0.004894497024657645,0.00011334911802145448
0.466,0.004603709434256204,0.00493855966442865,0.00011406908633928909
0.467,0.0046477994052413025,0.004982938735407757,0.00011479737761159039
0.468,0.0046922095590335566,0.005027636002735723,0.00011553966512180772
0.46900000000000003,0.00473694167169877,0.005072653239538054,0.00011629200874690742
0.47000000000000003,0.0047819975273462175,0.005117992226962132,0.00011705364633785081
0.47100000000000003,0.004827378918166204,0.005163654754214114,0.00011782486808889507
0.47200000000000003,0.004873087644467338,0.0052096426185965165,0.00011860649433455515
0.47300000000000003,0.004919125514714302,0.005255957625545879,0.00011940199083495707
0.47400000000000003,0.004965494345565931,0.005302601588670505,0.00012021824712690448
0.47500000000000003,0.005012195961913021,0.0053495763297886035,0.00012104954886086354
0.47600000000000003,0.0050592386305880884,0.0053968836789665174,0.00012189116606781224
0.47700000000000004,0.005106611343160098,0.005444525474557221,0.00012274688803288973
0.47800000000000004,0.005154322365706162,0.005492503563239082,0.00012362216971535116
0.47900000000000004,0.0052023735564316565,0.005540819800054792,0.00012451109208060098
0.48000000000000004,0.005250766781968326,0.005589476048450519,0.000125413962579187
0.481,0.0052995039174134695,0.0056384741803154285,0.00012633361312085417
0.482,0.005348586846369811,0.00568781607602104,0.00012726622680394383
0.483,0.00539801746098534,0.0057375036244613434,0.000128208091457233
0.484,0.00544779766199369,0.00578753872309281,0.0001291621902853618
0.485,0.005497929358754287,0.005837923277974734,0.00013012350261703727
0.486,0.0055484210786482385,0.005888659203809655,0.00013109214112580914
0.487,0.005599261547425388,0.005939748423984344,0.0001320703559855681
0.488,0.005650459292225531,0.005991192870610769,0.0001330591950935742
0.489,0.005702016257320503,0.006042994484567171,0.00013406933883187297
0.49,0.005753934395813974,0.006095155215539919,0.0001351054123549635
0.491,0.005806215669682671,0.006147677022064937,0.00013615733584787897
0.492,0.0058588620498188975,0.006200561871569932,0.00013722720059389148
0.493,0.005911875516072682,0.006253811740416457,0.00013830889393895142
0.494,0.005965258057294295,0.006307428613942515,0.00013940396363160075
0.495,0.006019011671377273,0.006361414486505192,0.0001405102497891536
0.496,0.006073145153247005,0.006415771361523755,0.00014163243589672826
0.497,0.006127646961144157,0.006470501251522805,0.00014276996122783217
0.498,0.006182525890304026,0.006525606178175721,0.00014392562793113058
0.499,0.00623778397522609,0.006581088172348485,0.00014510039889984114
0.5,0.00629342325967068,0.006636949274143661,0.0001462956435511517
0.501,0.006349445796703699,0.006693191532944644,0.0001475106111915891
0.502,0.006405853648740913,0.006749817007460107,0.0001487366816456362
0.503,0.006462648887592915,0.006806827765768888,0.00014997481474882818
0.504,0.0065198335945105355,0.006864225885364956,0.0001512338609289302
0.505,0.006577409860229717,0.006922013453202646,0.0001525140552077411
0.506,0.006635386754566937,0.006980192565742434,0.00015381007278333274
0.507,0.006693752466597969,0.0070387653289965815,0.00015512741102679953
0.508,0.006752516067040503,0.007097733858575299,0.00015646760122871447
0.509,0.006811679685031605,0.007157100279733072,0.00015782138733313238
0.51,0.006871245459424984,0.007216866727415515,0.00015919726692526024
0.511,0.0069312155388375415,0.00727703534630601,0.00016059445255222124
0.512,0.006991592081697005,0.007337608290873127,0.00016201690327720376
0.513,0.007052377256289613,0.007398587725417981,0.0001634695808588201
0.514,0.007113573240807633,0.007459975824122079,0.00016494330123654344
0.515,0.007175182223397746,0.007521774771095295,0.00016643744527220118
0.516,0.007237213556484632,0.007583986760424204,0.00016795096989790902
0.517,0.007299655158367519,0.007646613996220809,0.00016948775231906752
0.518,0.007362516383006826,0.007709658692671266,0.00017104842578840568
0.519,0.007425799458854189,0.007773123074085217,0.00017262695933769094
0.52,0.0074895066245603634,0.007837009374945187,0.00017423041490980464
0.521,0.007553640129025525,0.00790131983995648,0.00017586266284985215
0.522,0.007618202231449197,0.007966056724097047,0.00017751563266128168
0.523,0.007683195201381169,0.008031222292668113,0.00017919236503228622
0.524,0.007748621318771698,0.008096818821344652,0.0001808867727910156
0.525,0.007814482874022956,0.00816284859622642,0.00018260770358140377
0.526,0.007880789510277708,0.0082293139138893,0.00018435065131625704
0.527,0.007947528873500238,0.008296217081436802,0.00018610916750765304
0.528,0.008014710609050022,0.008363560416551952,0.00018788549616981397
0.529,0.008082337049653804,0.008431346247549555,0.0001896860811845599
0.53,0.008150410538749991,0.008499576913428713,0.00019151161144376737
0.531,0.00821893343054172,0.008568254763925505,0.0001933557332476425
0.532,0.0082879080900505,0.008637382159566371,0.000195219947206245
0.533,0.00835733689316923,0.008706961471721371,0.00019711049146147193
0.534,0.008427222226716383,0.008776995082658029,0.00019902956814966743
0.535,0.008497566488490215,0.008847485385595509,0.00020098199586799997
0.536,0.008568379620877024,0.008918434784758896,0.00020295947109975088
0.537,0.00863964899601201,0.008989845695434165,0.00020495904670086873
0.538,0.008711384559229275,0.009061720544023058,0.0002069830938347095
0.539,0.008783588752794941,0.009134061768098582,0.00020903689420100378
0.54,0.008856264030231096,0.009206871816460788,0.00021111910276473385
0.541,0.00892941285637173,0.009280153149192854,0.00021322417592882032
0.542,0.009003037707419649,0.009353908237717512,0.00021535548729741962
0.543,0.009077141071002878,0.009428139564853704,0.00021750919012311864
0.544,0.009151725446232209,0.009502849624873869,0.0002196953720054343
0.545,0.009226793343758654,0.009578040923561243,0.00022190882171145012
0.546,0.009302355014177477,0.009653715978267788,0.00022414960202930346
0.547,0.009378397554377771,0.009729877317972205,0.00022642572798961292
0.548,0.00945493121868733,0.009806527483338599,0.00022872751447686746
0.549,0.009531958564501173,0.009883669026775139,0.00023105565964740238
0.55,0.009609482161047836,0.009961304512493526,0.00023340883893674272
0.551,0.009687504589448875,0.010039436516568297,0.00023578956256602054
0.552,0.009766028442779358,0.01011806762699698,0.00023819991127191334
0.553,0.009845056326127727,0.010197200443760226,0.00024064097456413434
0.554,0.009924590856656913,0.010276837578882642,0.00024311282427656795
0.555,0.010004634663665685,0.010356981656493663,0.0002456077917987748
0.556,0.010085198315390703,0.010437635312889073,0.00024813386857291345
0.557,0.010166268632147566,0.010518801196592775,0.0002506879960326543
0.558,0.010247856186748333,0.010600481968418897,0.0002532797536808159
0.559,0.0103299636576534,0.010682680301534455,0.0002558976734290874
0.56,0.010412593735770281,0.010765398881522071,0.00025854409454263206
0.561,0.010495749124517314,0.010848640406443465,0.0002612214620670208
0.562,0.010579432539886965,0.010932407586903085,0.00026392960864441036
0.5630000000000001,0.010663646710510491,0.01101670314611215,0.00026666627068063826
0.5640000000000001,0.01074839437772219,0.011101529819953371,0.00026943502040330285
0.5650000000000001,0.010833678295625083,0.011186890357045414,0.0002722335882306944
0.5660000000000001,0.01091950936002604,0.011272787518808426,0.0002750590324007376
0.5670000000000001,0.011005874113443479,0.011359224079529764,0.0002779141146495467
0.5680000000000001,0.011092783457165002,0.011446202826429958,0.00028079736002214074
0.5690000000000001,0.011180240197024856,0.011533726559729182,0.00028370745910918737
0.5700000000000001,0.011268247151956574,0.011621798092714268,0.00028664389929351764
0.5710000000000001,0.011356807154060952,0.011710420251805876,0.0002896155382908224
0.5720000000000001,0.011445923048673212,0.011799595876626367,0.0002926222921828542
0.5730000000000001,0.01153559769443161,0.011889327820067786,0.0002956599361075705
0.5740000000000001,0.011625833963346485,0.011979618948360643,0.0002987300733356908
0.5750000000000001,0.011716634740868795,0.012070472141142536,0.0003018329762677709
0.5760000000000001,0.011808011260831284,0.01216189029152806,0.00030496540679935
0.5770000000000001,0.011899949786851981,0.012253876306178222,0.00030813462202847994
0.578,0.011992461559217057,0.012346433105371089,0.00031134611123401066
0.579,0.012085549517841099,0.012439563623071971,0.0003145895439573228
0.58,0.012179216616432382,0.012533270807005234,0.00031787201884779764
0.581,0.012273465822563745,0.01262755761872545,0.00032119559152588955
0.582,0.012368300117745114,0.012722427033689587,0.00032455399030740677
0.583,0.012463722497496063,0.012817882041329517,0.00032794721767168193
0.584,0.012559735971419383,0.012913925645124962,0.0003313837478742334
0.585,0.012656343563273866,0.013010560862676818,0.0003348658004683303
0.586,0.012753556855933584,0.013107790725781082,0.0003384172125602001
0.587,0.012851361833151127,0.013205618280503177,0.00034200984834491027
0.588,0.012949770085299397,0.0133040465872527,0.0003456423327084536
0.589,0.013048784693507922,0.013403078720858733,0.0003493306434660176
0.59,0.013148408753437655,0.013502717770645456,0.00035306627200378123
0.591,0.013248645375356864,0.013602966840508587,0.0003568443241086558
0.592,0.013349497684218182,0.01370382904899176,0.00036066285220823235
0.593,0.013450968819736382,0.013805307529363917,0.0003645220416392329
0.594,0.013553061936465384,0.01390740542969686,0.0003684259317019723
0.595,0.013655780203877182,0.014010125912943339,0.0003723757026320088
0.596,0.013759135565499127,0.014113472157015876,0.0003763645903545492
0.597,0.013863113724410544,0.01421744735486565,0.00038038954103172514
0.598,0.013967726632761655,0.014322054714562283,0.0003844565983755061
0.599,0.014072977520489386,0.014427297459373897,0.0003885759753956529
0.6,0.014178869632847193,0.014533178827847843,0.00039273744737226694
0.601,0.01428540623048694,0.01463970207389165,0.00039694016324219605
0.602,0.014392590589540491,0.014746870466854928,0.00040119245848597876
0.603,0.014500426001702335,0.014854687291611313,0.0004054968860791532
0.604,0.014608915774312137,0.014963155848641453,0.00040985333953866466
0.605,0.014718063230438306,0.015072279454115833,0.000414263903774895
0.606,0.014827880686508518,0.015182061439978904,0.00041872385049185893
0.607,0.014938353564300007,0.01529250515403327,0.00042323572542276867
0.608,0.015049494190072461,0.015403613960024315,0.0004278005223364944
0.609,0.015161305950654399,0.015515391237725752,0.00043242336149207334
0.61,0.01527379224902784,0.015627840383025542,0.0004370924526297081
0.611,0.015386956504415393,0.01574096480801233,0.0004418076946098395
0.612,0.01550080215236721,0.01585476794106231,0.000446582898623003
0.613,0.015615332644849234,0.015969253226926997,0.000451415633422826
0.614,0.015730551450330844,0.01608442412682125,0.0004562944977799576
0.615,0.01584646205387402,0.016200284118511994,0.0004612304217702599
0.616,0.015963077157731403,0.01631683669640739,0.0004662346796677612
0.617,0.016080381901951442,0.016434085371646853,0.00047130033502855103
0.618,0.01619838899991964,0.01655203367219129,0.0004764227588913584
0.619,0.016317102003969217,0.016670685142914234,0.0004816069048401946
0.62,0.016436524483479265,0.016790043345693225,0.00048685528369475824
0.621,0.016556660024966734,0.016910111859502187,0.0004921595421322188
0.622,0.016677512232180152,0.017030894280504145,0.0004975186179563425
0.623,0.016799084726192355,0.017152394222144485,0.0005029292101628659
0.624,0.01692138114549514,0.017274615315245028,0.0005083882444260401
0.625,0.017044405146093726,0.017397561208098582,0.0005138960925798897
0.626,0.017168169829712265,0.017521235566564042,0.0005194619999508781
0.627,0.01729266005447306,0.017645642074162315,0.0005250801817644388
0.628,0.017417888934633405,0.017770784432172768,0.0005307528643714667
0.629,0.01754386019721339,0.017896666359730026,0.0005364835328698779
0.63,0.01767057758723042,0.018023291593922016,0.0005422680154262477
0.631,0.017798044867796733,0.018150663889888046,0.0005481177587773259
0.632,0.01792626582021985,0.018278787020917762,0.0005540214956658951
0.633,0.018055244244101314,0.01840766477855086,0.0005599949119425526
0.634,0.018184983957437336,0.018537300972677372,0.0005660413746222563
0.635,0.018315488796720826,0.01866769943163832,0.0005721602782535335
0.636,0.018446772277565446,0.0187988640023276,0.00057833348912855
0.637,0.018578818976227762,0.018930798550294038,0.0005845614211868903
0.638,0.018711642422362385,0.019063506959844212,0.0005908478476708183
0.639,0.018845246527470844,0.019196993134146342,0.0005971981845828107
0.64,0.018979635222066093,0.019331260995334235,0.000603606859267814
0.641,0.01911481245577847,0.019466314484612196,0.0006100914786326959
0.642,0.019250782197460566,0.019602157562361052,0.0006166388542415778
0.643,0.019387548435294576,0.019738794208244086,0.0006232660713616628
0.644,0.019525115176899067,0.019876228421314195,0.0006299546069092438
0.645,0.019663486449437495,0.02001446422012159,0.000636705675973455
0.646,0.019802676197657545,0.020153505642822464,0.0006435195996312731
0.647,0.0199426687162985,0.020293356747287716,0.000650396825100389
0.648,0.020083477965772943,0.02043402161121316,0.0006573411448933869
0.649,0.02022510805251663,0.020575504332230148,0.0006643464225884532
0.65,0.020367563103060562,0.020717809028016714,0.0006714150380998405
0.651,0.02051084726414351,0.020860939836409766,0.0006785489138499716
0.652,0.020654964702824567,0.021004900915517877,0.0006857452053668315
0.653,0.02079991960659731,0.021149696443834947,0.0006930043837915375
0.654,0.020945716183504732,0.021295330620354307,0.0007003269234924044
0.655,0.02109235866225386,0.021441807664684235,0.0007077133020864035
0.656,0.02123986143285309,0.021589131817163244,0.0007151676347008214
0.657,0.021388208509197575,0.02173730733897721,0.0007226901690266318
0.658,0.021537414298710745,0.021886338512276483,0.000730283805061281
0.659,0.02168748311392639,0.022036229640294173,0.0007379480007728334
0.66,0.021838419288631488,0.022186985047465222,0.0007456859512731806
0.661,0.021990227177985558,0.022338609079546042,0.0007535025836803263
0.662,0.02214291115864191,0.022491106103735153,0.0007614225102249217
0.663,0.022296475628869127,0.022644480508794605,0.000769430948119511
0.664,0.022450925008674006,0.022798736705172122,0.000777517482347848
0.665,0.02260626373992412,0.022953879125124275,0.0007856779639842717
0.666,0.022762506674960697,0.02310991222284019,0.0007939146001721514
0.667,0.022919637547871137,0.023266840474566182,0.0008022229045377075
0.668,0.023077671230298767,0.023424668378731653,0.0008106160107899176
0.669,0.023236612252805818,0.02358340045607503,0.0008190886505786975
0.67,0.023396465168445367,0.023743041249771276,0.0008276372538527116
0.671,0.0235572345528887,0.02390359532555991,0.000836263290494331
0.672,0.023718925004555143,0.024065067271873918,0.0008449698496023495
0.673,0.02388154114474209,0.024227461699969734,0.000853753618129364
0.674,0.024045087617756342,0.024390783244057943,0.0008626127338771261
0.675,0.024209569091045303,0.024555036561434554,0.0008715625371078545
0.676,0.02437500089736909,0.02472022633261404,0.0008806058929011375
0.677,0.02454136649244944,0.024886357261462433,0.0008897453171941064
0.678,0.02470868123038396,0.025053434075331497,0.0008989629528283053
0.679,0.024876949872521724,0.025221461525194402,0.0009082657412371536
0.68,0.02504617720402572,0.025390444385781617,0.0009176780433276694
0.681,0.025216368034010558,0.025560387455717818,0.0009271916103279905
0.682,0.02538752719568056,0.02573129555766024,0.0009367930072433121
0.683,0.025559659546469646,0.025903173538437435,0.0009464797773939766
0.684,0.025732769968180698,0.026076026269189354,0.0009562608866587189
0.685,0.025906863367127327,0.026249858645508106,0.0009661252859255912
0.686,0.026081955575662334,0.0264246755875798,0.0009760751357571466
0.687,0.026258029773037365,0.026600482040327545,0.0009861151554479725
0.6880000000000001,0.026435101815139427,0.026777282973554948,0.0009962406969026224
0.6890000000000001,0.026613176707756505,0.026955083382091398,0.0010064583939100363
0.6900000000000001,0.026792259481907544,0.027133888285937376,0.0010167626717399554
0.6910000000000001,0.026972355193990192,0.027313702730411324,0.001027169247444006
0.6920000000000001,0.027153468925928577,0.027494531786297922,0.0010376757826750357
0.6930000000000001,0.027335605785322636,0.02767638054999648,0.0010482770376624415
0.6940000000000001,0.027518770905598577,0.02785925414367085,0.0010589704762556445
0.6950000000000001,0.027702969446159402,0.028043157715400613,0.0010697541454629882
0.6960000000000001,0.027888217759293527,0.02822809643933277,0.0010806287107079956
0.6970000000000001,0.028074498750182954,0.02841407551583501,0.0010915948419507459
0.6980000000000001,0.028261828797022204,0.02860110017164949,0.001102653213718635
0.6990000000000001,0.02845021316465757,0.02878917566004825,0.0011138281664979874
0.7000000000000001,0.028639657144684992,0.028978307260989506,0.0011251055583693962
0.7010000000000001,0.028830166055607245,0.02916850028127459,0.001136477615003135
0.7020000000000001,0.02902174524299375,0.02935976005470685,0.0011479450324900326
0.7030000000000001,0.029214400079639328,0.029552091942250985,0.0011595085116662483
0.7040000000000001,0.02940813596572575,0.02974550133219352,0.001171169064549379
0.705,0.029602958328983985,0.029939993640305168,0.0011829334113444179
0.706,0.029798884063236476,0.030135574310002692,0.0011947960275321343
0.707,0.029995895802560634,0.030332248812514326,0.0012067576338613854
0.708,0.030194010469247717,0.030530022647044075,0.0012188189559942898
0.709,0.030393233602869447,0.030728901340938097,0.0012309807245395826
0.71,0.03059357077137492,0.030928890449852857,0.0012432469512662736
0.711,0.030795027571259,0.031129995557923302,0.0012556156094483493
0.712,0.03099760962773367,0.03133222227793295,0.0012680869794246899
0.713,0.03120132259489846,0.031535576251485266,0.001280661812275792
0.714,0.03140617215591377,0.031740063149175685,0.0012933408642022662
0.715,0.03161216402317505,0.03194568867076526,0.0013061477704989217
0.716,0.03181931565499017,0.03215245854535556,0.0013190834206316905
0.717,0.032027609417924575,0.03236037853156469,0.00133212915827617
0.718,0.03223706280152508,0.032569454417704494,0.0013452827559414754
0.719,0.03244768163689031,0.03277969202195909,0.001358545722653868
0.72,0.03265947178524253,0.032991097192564885,0.0013719238803891224
0.721,0.03287243913810879,0.03320367580799154,0.0013854123475164279
0.722,0.03308658961750351,0.03341743377712425,0.0013990122290646833
0.723,0.03330192917611281,0.03363237703944786,0.0014127293240194063
0.724,0.03351846379748017,0.03384851156523137,0.0014265592189020657
0.725,0.03373619949619297,0.034065843355714734,0.0014405027343707558
0.726,0.033955154319453125,0.03428437844329617,0.0014545686312080238
0.727,0.0341753103706062,0.03450412289172155,0.0014687499032749124
0.728,0.03439668573108865,0.03472508279627444,0.0014830473830738354
0.729,0.03461928654155861,0.03494726428396824,0.0014974619146104627
0.73,0.03484311897467187,0.03517067351373885,0.001511998081422003
0.731,0.03506818923527812,0.03539531667663982,0.001526661524361866
0.732,0.0352945035606159,0.03562119999603762,0.0015414523464081626
0.733,0.035522068220511224,0.035848329727809644,0.0015563644778551157
0.734,0.03575088951757647,0.03607671216054259,0.001571399972858599
0.735,0.03598097378741161,0.036306353615732576,0.0015865646359972028
0.736,0.03621233969209321,0.03653726044798748,0.001601859622205815
0.737,0.036444969076816075,0.03676943904522932,0.0016172790337252573
0.738,0.03667888064113362,0.03700289582889932,0.0016328237710471014
0.739,0.03691408085463081,0.03723763725416379,0.0016484991834513631
0.74,0.03715057622090559,0.037473669810122116,0.0016643256137198288
0.741,0.03738837327777817,0.03771100002001556,0.0016802957017256865
0.742,0.03762747859750224,0.037949634441437896,0.0016964004594051821
0.743,0.03786789878697757,0.03818957966654799,0.001712635653000584
0.744,0.038109640487964655,0.03843084232228286,0.0017290022244566036
0.745,0.03835271037729968,0.03867342907057388,0.0017455011221549287
0.746,0.03859712775961122,0.03891734660856296,0.001762136765279964
0.747,0.03884287422787957,0.039162601668821316,0.0017789079070458654
0.748,0.03908996912772116,0.03940920101956993,0.0017958143118035658
0.749,0.039338419278467415,0.039657151464900425,0.0018128581926696156
0.75,0.03958823153562968,0.03990645984499922,0.0018300519689252845
0.751,0.03983941279112355,0.040157133036372084,0.0018473861674715383
0.752,0.040091969973497156,0.04040917795207125,0.0018648733757690083
0.753,0.040345910048158865,0.040662601541923096,0.0018825045662334934
0.754,0.04060124001760922,0.04091741079275867,0.0019002773238568913
0.755,0.040857966921672,0.041173612728645656,0.001918192667035953
0.756,0.04111611073703943,0.0414312144111209,0.0019362516211381836
0.757,0.041375652811376604,0.04169022293942688,0.001954461097483825
0.758,0.04163661316616828,0.041950645450747726,0.0019728224152749997
0.759,0.04189899899289132,0.04221248912044789,0.0019913374389952474
0.76,0.04216281752153362,0.04247576116231345,0.002010000455765896
0.761,0.042428076020836744,0.042740468828793954,0.002028821160592212
0.762,0.04269478179854165,0.043006619411245936,0.002047798915435802
0.763,0.04296294220163447,0.043274220240180024,0.0020669365533101556
0.764,0.043232564616594575,0.04354327868550787,0.0020862267554731142
0.765,0.043503656469645414,0.04381380215679201,0.0021056706024227484
0.766,0.04377623844104031,0.044085798103497206,0.002125269195707367
0.767,0.04405029164110029,0.044359274015244324,0.002145023644430878
0.768,0.04432583679899656,0.04463423742206547,0.0021649350653062706
0.769,0.044602881502468765,0.044910695894660624,0.002185004582709406
0.77,0.044881433380278654,0.04518865704465777,0.0022052333287333275
0.771,0.045161500102473676,0.045468128524873266,0.002225622443242919
0.772,0.045443089380649615,0.04574911802957552,0.002246173073929987
0.773,0.04572620896821745,0.04603163329474965,0.0022668863763688455
0.774,0.04601086666066994,0.04631568209836476,0.0022877635140723077
0.775,0.04629707029585149,0.046601272260643506,0.0023088056585480275
0.776,0.04658484129122583,0.046888411644332315,0.0023300139893554332
0.777,0.04687416052893186,0.04717710815497571,0.002351389694162998
0.778,0.04716504947982851,0.047467369741190854,0.002372933968805994
0.779,0.04745751615390765,0.04775920439494559,0.00239464801734477
0.78,0.04775156860489337,0.04805262015183754,0.0024165330521233263
0.781,0.04804721493052357,0.04834762509137593,0.0024386002575954306
0.782,0.04834446327283571,0.048644227337265644,0.0024608412100057264
0.783,0.04864332181845205,0.048942435057693225,0.00248326435163827
0.784,0.04894379879886944,0.0492422564656146,0.002505874288882506
0.785,0.049245902490749914,0.049543699819046216,0.002528692449976796
0.786,0.04954965508474766,0.04984677342135738,0.0025517402421395283
0.787,0.049855037245311526,0.05015148562156515,0.002574972455418212
0.788,0.05016207122135271,0.05045784481463183,0.002598399147940218
0.789,0.05047076547315144,0.05076585944176407,0.002622009490383969
0.79,0.050781128507643554,0.05107553799071482,0.002645804791765313
0.791,0.05109316887872417,0.0513868889960879,0.002669786370134059
0.792,0.051406895187556194,0.05169992103964387,0.0026939555526390986
0.793,0.05172231608287824,0.05201464275060945,0.002718313675593982
0.794,0.05203944026131825,0.052331062805988454,0.002742864938692541
0.795,0.0523582764677068,0.052649189930875896,0.0027676315052622322
0.796,0.05267884770440448,0.05296903289877364,0.0027925955057288574
0.797,0.05300113443013614,0.0532906005319096,0.002817754216311639
0.798,0.053325159710802525,0.05361390170155829,0.0028431090226844077
0.799,0.053650932487241045,0.05393894532836489,0.0028686613201077374
0.8,0.053978461750101285,0.054265740382671526,0.002894412513498452
0.801,0.05430775654017519,0.054594295884845156,0.0029203640174996176
0.802,0.054638825948728445,0.05492462090561007,0.002946517256551216
0.803,0.054971679117835466,0.05525672456638082,0.002972873664961208
0.804,0.055306325240716485,0.05559061603959913,0.002999434686977339
0.805,0.05564277356207827,0.05592630454907338,0.003026201776859458
0.806,0.0559810479372568,0.0562637993703196,0.0030531797246292165
0.807,0.05632112863286516,0.05660310983090725,0.0030803948805254266
0.808,0.056663039573526135,0.0569442453108054,0.003107820834250528
0.809,0.05700679021334418,0.057287215242733516,0.003135459083128628
0.81,0.05735239005964939,0.05763202911251379,0.0031633111348821734
0.811,0.05769984867335592,0.057978696459427194,0.0031913785077079754
0.812,0.05804917566931921,0.05832722687657128,0.0032196893349885044
0.8130000000000001,0.05840038071669934,0.058677630011222205,0.003248224922114984
0.8140000000000001,0.05875347353932523,0.0590299155651988,0.003277010220591005
0.8150000000000001,0.05910846391606404,0.05938409329522902,0.0033060176775010393
0.8160000000000001,0.05946537659949776,0.059740173013320685,0.003335248869564303
0.8170000000000001,0.05982419167956827,0.060098164587134045,0.0033647077224390936
0.8180000000000001,0.06018493398439946,0.060458077940357846,0.0033944055798534266
0.8190000000000001,0.06054761351674534,0.06081992305308835,0.003424332122498099
0.8200000000000001,0.06091224033628205,0.061183709962211355,0.003454488972670544
0.8210000000000001,0.061278824559992624,0.061549448761787626,0.00348487776398222
0.8220000000000001,0.061647376362556724,0.06191714960344,0.0035155001414420265
0.8230000000000001,0.062017905976743025,0.06228682269674616,0.0035463577615405693
0.8240000000000001,0.06239042369380403,0.06265847830963236,0.00357747413132286
0.8250000000000001,0.06276493986387528,0.06303212676877083,0.003608842790798229
0.8260000000000001,0.06314148018432486,0.06340777845998107,0.0036404521040483543
0.8270000000000001,0.06352002458590411,0.06378544382863445,0.0036723037771698853
0.8280000000000001,0.0639005988483368,0.06416513338006076,0.0037043995281926447
0.8290000000000001,0.0642832135613405,0.06454685767995917,0.0037367410871683667
0.8300000000000001,0.06466787937555779,0.06493062735481273,0.003769330196260027
0.8310000000000001,0.06505460700297412,0.06531645309230584,0.003802168609831965
0.8320000000000001,0.06544340721733943,0.0657043456417442,0.0038352580945408376
0.8330000000000001,0.06583429085459434,0.06609431581448012,0.0038686004294272184
0.834,0.06622726881329882,0.06648637448434006,0.0039021974060078793
0.835,0.06662235205506295,0.06688053258805517,0.003936050828369574
0.836,0.06701956727314914,0.06727680112569745,0.0039701625132621534
0.837,0.06741889425887305,0.06767519116111699,0.004004534290193904
0.838,0.06782035979528223,0.0680757138223844,0.004039168001526964
0.839,0.06822397510058706,0.06847838030223594,0.00407406550257371
0.84,0.06862975145826299,0.06888320185852413,0.004109228661693943
0.841,0.06903770021750696,0.06929018981466933,0.00414465936039291
0.842,0.06944783279369304,0.06969935556011703,0.00418035949342009
0.843,0.06986016066883614,0.07011071055079841,0.00421633096886894
0.844,0.07027469539205557,0.07052426630959485,0.0042525757082773515
0.845,0.07069144858004524,0.07094003442680602,0.0042890956467291205
0.846,0.07111044797697087,0.07135802656062185,0.004325892732956087
0.847,0.07153167325700245,0.07177825443759854,0.00436297770021718
0.848,0.07195515226220013,0.07220072985313868,0.004400345786725313
0.849,0.07238089688432742,0.0726254646719753,0.0044379970628804855
0.85,0.07280891908512778,0.07305247082865995,0.004475933533903506
0.851,0.07323923089681823,0.07348176032805458,0.004514157219193674
0.852,0.07367184442258658,0.07391334524582795,0.004552670152436543
0.853,0.07410677183709259,0.07434723772895613,0.004591486099256422
0.854,0.07454402538697417,0.07478344999622676,0.004630598669207248
0.855,0.07498361739135767,0.07522199433874865,0.004670006830735508
0.856,0.0754255767045908,0.07566288312046388,0.004709712676948651
0.857,0.07586988290881805,0.0761061287786666,0.004749718315801038
0.858,0.07631656496513944,0.07655174382452366,0.004790025870207138
0.859,0.07676563548782103,0.0769997408436013,0.004830637478156036
0.86,0.07721710716623217,0.0774501324963962,0.0048715552928267035
0.861,0.07767099276538193,0.0779029315188707,0.004912781482704366
0.862,0.07812730512646074,0.07835815072299149,0.0049543182316978875
0.863,0.078586057167385,0.07881580299727588,0.004996167739258105
0.864,0.07904726188334901,0.07927590130733912,0.005038332220497293
0.865,0.07951093234737759,0.0797384586964487,0.005080813906309607
0.866,0.07997709858795991,0.08020348828608316,0.0051236150434925895
0.867,0.08044574012349416,0.08067100327649496,0.005166737894869638
0.868,0.08091688709890801,0.0811410169472774,0.005210184739413801
0.869,0.08139055290419962,0.08161354265794021,0.005253957872372381
0.87,0.08186675101004594,0.08208859384848413,0.005298059605392798
0.871,0.08234549496838602,0.0825661840399867,0.005342492266649462
0.872,0.08282679841301165,0.08304632683518733,0.00538725820097184
0.873,0.08331067506016009,0.08352903591908228,0.005432359769973665
0.874,0.08379713870911427,0.08401432505952142,0.005477799352183071
0.875,0.0842862032428069,0.08450220810781196,0.00552358656320414
0.876,0.08477789993296254,0.0849926989993268,0.005569721498714629
0.877,0.0852722082660462,0.08548581175411785,0.005616201809785603
0.878,0.08576915964082364,0.08598156047753533,0.005663044627098699
0.879,0.08626876828097875,0.08647995936085211,0.005710241490056055
0.88,0.08677104849694753,0.08698102268189323,0.005757791296482397
0.881,0.08727601468655606,0.08748476480567186,0.005805736242290836
0.882,0.08778368133566061,0.08799120018502929,0.005854044564009348
0.883,0.08829406301879757,0.08850034336128217,0.005902713862624395
0.884,0.08880717439983525,0.0890122089648741,0.0059517466991316015
0.885,0.08932303023263526,0.0895268117160338,0.006001145652995537
0.886,0.08984166310689841,0.09004416642543872,0.006050913322295101
0.887,0.0903630525129206,0.09056428799488407,0.006101052323869882
0.888,0.09088723117906126,0.0910871914179592,0.006151565293468149
0.889,0.09141421422586125,0.09161289178072735,0.006202454885895924
0.89,0.09194401686723812,0.09214140426241488,0.006253723775167562
0.891,0.09247665441118268,0.0926727441361027,0.006305374654657527
0.892,0.093012142260458,0.0932069267694277,0.006357410237253766
0.893,0.09355049591330769,0.09374396762528714,0.006409833255512237
0.894,0.09409173096417,0.0942838822625514,0.0064626464618129575
0.895,0.09463586310439775,0.09482668633678232,0.006515852628517438
0.896,0.09518292632262575,0.09537239560095787,0.00656945454812759
0.897,0.09573290015316807,0.09592102590620301,0.006623464653852707
0.898,0.09628581873606143,0.09647259320252874,0.006677912186037443
0.899,0.09684169815764582,0.0970271135395742,0.006732764443464725
0.9,0.09740055460487355,0.09758460306736051,0.00678802430445587
0.901,0.09796240436606853,0.098145078037047,0.00684369466831556
0.902,0.09852726383169227,0.09870855480169555,0.006899778455499829
0.903,0.09909514949511775,0.09927504981704294,0.0069562786077856185
0.904,0.09966607795340963,0.09984457964227968,0.007013198088441725
0.905,0.10024006590811112,0.10041716094083376,0.007070539882401498
0.906,0.10081714883460305,0.1009928104811646,0.007128306996437125
0.907,0.10139730635636221,0.10157154513756333,0.007186502459335361
0.908,0.10198057411416596,0.10215338189095864,0.007245129322075015
0.909,0.10256696923548983,0.10273833782973128,0.007304190658005961
0.91,0.10315650895633313,0.10332643015053634,0.007363689563030029
0.911,0.10374921062205021,0.10391767615913255,0.007423629155783306
0.912,0.10434509168818765,0.10451209327121912,0.007484012577820237
0.913,0.1049441697213335,0.105109699013279,0.007544842993799525
0.914,0.10554646239996883,0.10571051102343326,0.00760612359167164
0.915,0.10615198751533117,0.1063145470522991,0.007667857582868045
0.916,0.10676078212492943,0.10692182496385905,0.007730048202492322
0.917,0.10737282599210919,0.10753236273633598,0.007792698709513056
0.918,0.10798815635516293,0.10814617846307861,0.007855812386958361
0.919,0.10860679146513223,0.1087632903534507,0.007919392542112408
0.92,0.10922874969024514,0.1093837167337348,0.007983494057478582
0.921,0.10985404951682694,0.11000747604803837,0.008048073619167227
0.922,0.11048270955021862,0.11063458685921271,0.008113130290334994
0.923,0.11111474851570613,0.11126506784977692,0.008178667481533928
0.924,0.11175018525945499,0.11189893782285273,0.008244688628613599
0.925,0.11238903874945588,0.11253621570310848,0.008311197192929361
0.926,0.11303134772910343,0.11317692053770917,0.008378196661552284
0.927,0.11367709215856443,0.11382107149727802,0.008445690547481309
0.928,0.1143263109789538,0.11446868787686496,0.008513682389857119
0.929,0.11497902365519391,0.11511978909692752,0.008582175754178419
0.93,0.11563524977889035,0.11577439470431547,0.008651174232519914
0.931,0.11629500906933381,0.11643252437327037,0.008720681443752655
0.932,0.11695832137450692,0.11709419790643118,0.008790701033766264
0.933,0.11762520667210398,0.11775943523585022,0.008861236675693423
0.934,0.1182956850705574,0.11842825642401837,0.008932292070136474
0.935,0.11896977681007738,0.11910068166490055,0.00900387094539616
0.936,0.11964752243297967,0.11977673128498123,0.009075977057702545
0.937,0.12032890216022783,0.12045642574431861,0.00914861419144833
0.9380000000000001,0.12101395675052827,0.1211397856376096,0.009221786159424325
0.9390000000000001,0.12170270698177113,0.12182683169526537,0.009295496803056425
0.9400000000000001,0.12239517376895995,0.12251758478449627,0.009369749992646776
0.9410000000000001,0.12309137816531016,0.12321206591040733,0.009444549627615272
0.9420000000000001,0.12379134136335818,0.12391029621710518,0.009519899636744454
0.9430000000000001,0.12449508469608,0.12461229698881336,0.009595803978426458
0.9440000000000001,0.1252026296380212,0.1253180896510009,0.009672266640912525
0.9450000000000001,0.12591399780643794,0.12602769577152031,0.009749291642564861
0.9460000000000001,0.12662923166590875,0.126741137061756,0.00982695494008751
0.9470000000000001,0.12734831177007305,0.1274584353777861,0.009905338344904207
0.9480000000000001,0.12807128082050415,0.12817961272155143,0.009984298580872837
0.9490000000000001,0.128798161016931,0.12890469124204093,0.01006383980687284
0.9500000000000001,0.12952897470766397,0.12963369323648335,0.010143966213323691
0.9510000000000001,0.13026374439080363,0.1303666411515549,0.01022468202245294
0.9520000000000001,0.13100249271546124,0.13110355758459616,0.010305994723940672
0.9530000000000001,0.13174524248299063,0.13184446528484045,0.010387949155275076
0.9540000000000001,0.13249201664823182,0.13258938715465557,0.010470506319395041
0.9550000000000001,0.13324283832076647,0.1333383462507985,0.010553670572094801
0.9560000000000001,0.1339977520222316,0.1340913657856783,0.010637446302384569
0.9570000000000001,0.13475673871973526,0.13484846912863693,0.010721837932775044
0.9580000000000001,0.13551984319467916,0.1356096798072376,0.010806849919564843
0.9590000000000001,0.13628708918842725,0.13637502150856917,0.01089248675313078
0.9600000000000001,0.13705850060355368,0.13714451808056083,0.010978752958220936
0.961,0.13783410150517642,0.137918193533313,0.011065653094250588
0.962,0.13861391612229962,0.13869607204043743,0.011153267590694956
0.963,0.13939796884917477,0.13947817794041278,0.011241528146327805
0.964,0.14018628424667007,0.14026453573795575,0.01133043731595914
0.965,0.14097888704365824,0.141055170105399,0.011419999806878845
0.966,0.14177582396639055,0.14185010588409114,0.011510220362617162
0.967,0.14257707648629828,0.14264936808580447,0.011601103763259294
0.968,0.14338269161460002,0.14345298189415884,0.011692654825763246
0.969,0.1441926947663137,0.14426097266606175,0.011784878404281017
0.97,0.14500711153159576,0.1450733659331574,0.011877779390482866
0.971,0.1458259676772151,0.14589018740329718,0.011971362713884947
0.972,0.14664928914803407,0.1467114629620191,0.012065633342180181
0.973,0.14747710206851125,0.14753721867404548,0.012160596281572657
0.974,0.14830943274421496,0.1483674807847944,0.012256256577115194
0.975,0.14914630766335543,0.14920227572190584,0.01235261931305067
0.976,0.1499877759186089,0.1500416300967851,0.012449689613156357
0.977,0.1508338195879492,0.1508855707061605,0.012547472641092272
0.978,0.15168448807695112,0.15173412453365495,0.01264597360075282
0.979,0.1525398086200029,0.15258731875138007,0.012745197736621968
0.98,0.15339980864202163,0.15344518072153696,0.012845150334132341
0.981,0.15426451576007832,0.15430773799804087,0.012945836720027875
0.982,0.15513395778503883,0.15517501832815978,0.013047262262729937
0.983,0.1560081627232258,0.156047049654169,0.013149432372707803
0.984,0.15688715877809176,0.156923860115026,0.013252352502852312
0.985,0.15777097435191517,0.157805478048054,0.013356028148853982
0.986,0.15865966108154098,0.15869193199065545,0.013460464849584599
0.987,0.15955320176658,0.1595832506820324,0.013565668187482944
0.988,0.16045164838777937,0.1604794630649288,0.013671643788944591
0.989,0.16135503015999922,0.16138059828739248,0.013778397324715674
0.99,0.162263376505657,0.16228668570455113,0.013885934510290679
0.991,0.16317671705652656,0.16319775488041036,0.013994261106314713
0.992,0.16409508165555614,0.16411383558966885,0.014103382918989563
0.993,0.16501850035870957,0.16503495781955005,0.0142133058004843
0.994,0.1659470034368228,0.16596115177166057,0.014324035649350055
0.995,0.16688062137747844,0.16689244786385612,0.014435578410939396
0.996,0.16781940855729474,0.1678288767321396,0.014547940077829627
0.997,0.16876334862720782,0.16877046923256847,0.014661126690251157
0.998,0.169712496342207,0.1697172564431884,0.014775144336519956
0.999,0.1706668830760333,0.17066926966598625,0.014889999153474815
1.0,0.17162654042885994,0.17162654042885994,0.015005697326919098
